Unpacking How Decentralized Autonomous Organizations (DAOs) Work in Practice

Decentralized Autonomous Organizations (DAOs) have emerged as a novel way to coordinate a group of (pseudonymous) entities towards a shared vision (e.g., promoting sustainability), utilizing self-executing smart contracts on blockchains to support decentralized governance and decision-making. In just a few years, over 4,000 DAOs have been launched in various domains, such as investment, education, health, and research. Despite such rapid growth and diversity, it is unclear how these DAOs actually work in practice and to what extent they are effective in achieving their goals. Given this, we aim to unpack how (well) DAOs work in practice. We conducted an in-depth analysis of a diverse set of 10 DAOs of various categories and smart contracts, leveraging on-chain (e.g., voting results) and off-chain data (e.g., community discussions) as well as our interviews with DAO organizers/members. Specifically, we defined metrics to characterize key aspects of DAOs, such as the degrees of decentralization and autonomy. We observed CompoundDAO, AssangeDAO, Bankless, and Krausehouse having poor decentralization in voting, while decentralization has improved over time for one-person-one-vote DAOs (e.g., Proof of Humanity). Moreover, the degree of autonomy varies among DAOs, with some (e.g., Compound and Krausehouse) relying more on third parties than others. Lastly, we offer a set of design implications for future DAO systems based on our findings.

==> arxiv_2024_S&P_DAO-Paper_final/section/Discussion.tex <==
\vspace{-2mm}
\section{Discussion}
\vspace{-2mm}
\label{section7}
In this section, we discuss the prevailing governance structure of DAOs and the degree to which they realize their envisioned goals. Based on the current outcomes of DAOs, we also provide \emph{governance and design implications} of DAOs, and identify areas warranting further investigation.

\vspace{-2mm}
\subsection{Recap of Main Findings} 
\vspace{-2mm}
DAO represents a significant artifact for comprehending emerging forms of algorithmic authority, exploring practical modes of governance for autonomous and decentralized systems, and understanding the ways that designing incentives and modeling can fail~\cite{dupont2017experiments}. In our interview, DAO experts indicated three metrics including, token distribution, voter participation, and geographical distribution for decentralization, while some of these were evaluated in our subsequent empirical analysis to understand the impact in the decentralization level. Our constructed voting network graph for each DAO and calculated clustering and connectivity metrics show that there is a higher degree of voting pattern polarization of large token holders relative to other DAO members. We also found a significant positive correlation between the proposal’s author token balance and the proposal's success in some DAOs, which may be a bad sign in DAOs where voting power is traded on the secondary market. To quantify decentralization, we applied entropy, the Gini coefficient, and the Nakamoto coefficient of the token distribution and the voting participation rate of voters. We found that DAOs that allow governance tokens to be bought from the secondary market are less decentralized over time, contradicting the expectation of a DAO becoming more decentralized over time, while those adopting the one-person-one-vote protocol have increased decentralization.

In terms of autonomy, we explored the dependency of a DAO on external entities and the degree of intervention a DAO needs to carry out its actions. We found that many offchain DAOs use a Multisig wallet to translate the consensus reached offchain to onchain actions, resulting in lower autonomy.  Kleros Governor is an interesting alternative, but the method can lack autonomy as it relies on multi-step checks done after consensus.
The portion of proposals relying on third-party services after execution varies from 0-75\% among the DAOs studied. Another metric calculated in this study is the number of proposals canceled after voting ends. This metric is particularly important as it shows to what degree the community consensus is respected, however this analysis is constrained by the limited transparency of offchain DAOs. The large number of such proposals call for the need for more transparent proposal tracking tools.

%In this matter, DAO experts noted that the pods-like structure would facilitate autonomy among DAO members for different actions, such as finance, protocol, and engineering, however, this idea sounds like rebranded sub-committee rather than a novel structure. 
In summary, we provide an overall characterization of governance structures present in DAOs and assess their level of success. Subsequently, we delve into the extent to which the observed outcomes can be attributed to the design choices made in the DAOs, such as the role of marketing factors versus the impact of the governance process design. 
%In the next section, we provided design implications.

%Angles of autonomy explored in  this paper is the dependency of a DAO on external entities and the degree of intervention a DAO needs to carry out its actions. While many onchain DAOs have their proposal pipeline done onchain to ensure autonomy of proposal execution, many offchain DAOs use a Multisig wallet to translate the consensus reached offchain to onchain actions, resulting in poor autonomy. Kleros Governor is an interesting alternative, but the method can lack autonomy as it relies on multi-step checks done after consensus. Autonomy can also be explored on the proposal level as many DAO proposals rely on third-party services after execution to achieve the proposals' goal. Experts also suggested "pods" like structure to facilitate autonomy among DAO members with different actions, such as , finance, protocol, engineering, however this sounds like a hip euphemism for "sub-committee", pointing this out could be useful for the point that they are often rebranded structures rather than novel structures. The portion of proposals relying on third-party services after execution varies from 0-75\% among the DAOs studied. Another metric calculated in this study is the number of proposals canceled after voting ends. This metric is particularly important as it shows to what degree the community consensus is respected; however, some limitations of this analysis are the limited transparency of offchain DAOs and the large number of proposals indicating transparent proposal tracking tools. 

%We characterize the governance structures, and characterize their current level of success in current DAOs. In the next section, we discuss what degree the outcomes can be explained by the design choices (e.g., the outcome of whale token distribution could be caused in part by marketing factors vs due to the design of the governance process).
\vspace{-2mm}
\subsection{Design Implication}
\vspace{-2mm}
\noindent\textbf{Incentive mechanism: separation between voting power and monetary value.} 
%Healthy and robust DAOs are generally considered the ones in which many entities evenly participate. 
One of the most critical points that enable healthy and robust DAOs is facilitating equitable participation of numerous entities which necessitates proper incentive systems~\cite{argon}. Our paper confirmed that 
biased voting power distribution or low participation rate in many existing DAOs can be attributed to a lack of proper incentive system
%many existing DAOs struggle with a biased voting power distribution or a low participation rate, which implies that current DAOs lack proper incentive systems
~\cite{kaal2021decentralized}. Whereas DAO experts also suggested a separation between voting power and monetary value
%These suggest separating voting power from monetary values 
might be needed to achieve better decentralization. 
%These observations suggest that separating voting power from monetary values may result in better decentralization. 
Although the optimal incentive designs for decentralization are unclear, DAO practitioners can consider a handful of design choices to help address this issue. First, DAO practitioners can choose to have nontransferable/non-monetary vote tokens. They can consider social rewards like reputation, such as, reputation-based voting, and contribution-based voting, one person one vote. Some studies~\cite{liu2022user,guidi2020graph} showed that social rewards could be effective in promoting the engagement of users in the DAO context. Alternatively, DAOs with existing transferable voting tokens can choose to adopt a quadratic voting scheme, making the purchase of a unit voting power increasingly expensive as users hold more tokens.

%(especially, Proof of Humanity, MetaGammaDelta, and MolochDAO; please refer to Gini of the voting score and the number of voters in Table~\ref{tab:decen-level}), which hinders decentralization. 
%To address this, DAOs need better incentive systems for users to participate more actively in governance. 
%On the other hand, our findings also show that simply separating voting power from the monetary value does not necessarily result in a high decentralization level. 
%For example, Proof of Humanity and MetaGammaDelta, which do not adopt the monetary-based incentive approach, have suffered from a low number of active voters hindering decentralization. 


%Currently, many DAOs adopt a monetary-based incentive approach to attract many people. Even though this approach may be the most attractive to users, it causes bad decentralization bringing about biased voting power distribution.
%Specifically, we empirically observed a positive correlation between the voting power of proposers and proposal outcome. This raises concern that an individual could buy their power. Moreover, as individuals with larger voting power tend to participate more actively in voting, individuals with lower capital can be more underrepresented in DAOs where voting power is traded on the secondary market. Further, it is observed that DAOs that associate voting power with monetary value become less decentralized over time. %as opposed to their counterparts. 
%Indeed, the previous literature also proves that it is almost impossible to attain a high decentralization level in monetary-based incentive systems with an anonymous setting~\cite{kwon2019impossibility}. Some DAO experts also suggested a separation between voting power and monetary value. These suggest separating voting power from monetary values might be needed to achieve better decentralization. 



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%original version
\begin{comment}   
\noindent\textbf{Tokenomics of DAOs governance token.} It is an important topic regarding DAOs decentralization. One integral design choice is whether or not the governance token should be associated with monetary values. %In regards to decentralization, it is observed that a 
DAO experts suggested a separation between voting power and monetary value. We also empirically observed a positive correlation between the voting power of proposers and proposal outcome. This raises concern that an individual could buy their power. Moreover, as individuals with larger voting power tend to more actively participate in voting, individuals with lower capital can be more underrepresented in DAOs where voting power is traded on the secondary market. Most importantly, it is observed that DAOs that associate voting power with monetary value become less decentralized over time. %as opposed to their counterparts. 
Indeed, the previous literature also proves that it is almost impossible to attain a high decentralization level under an anonymous setting~\cite{kwon2019impossibility}. 
These observations suggest that separating voting power from monetary values may result in better decentralization. There are a handful of design choices that help address this issue. First, DAO practitioners can choose to have nontransferable vote tokens. Some examples of the such scheme include one person one vote, reputation-based voting, and contribution-based voting. Second, DAOs with existing transferable voting tokens can choose to adopt quadratic voting scheme, making the purchase of a unit voting power increasingly expensive as users hold more tokens.

\noindent\textbf{Incentives for participating in the voting. } The greater the number of active voters, the healthier DAO governance can be attained. However, as shown in our paper, some DAOs suffer from a low number of active voters (especially, Proof of Humanity, MetaGammaDelta, and MolochDAO; please refer to Gini of the voting score and the number of voters in Table~\ref{tab:decen-level}), which hinders decentralization. To address this, DAOs need incentive systems for users to more actively participate in governance. Currently, many DAOs adopt a monetary-based incentive approach. Even though this approach may be the most attractive to users, it again causes bad decentralization bringing about a biased voting power distribution.
%Therefore, DAOs would need better incentive systems 

In fact, it is unclear what the optimal incentive designs are in terms of decentralization
%, and even there has been yet little research on DAO incentives \cite{liu2022user}. 
Some studies \cite{liu2022user,guidi2020graph} show that not only monetary rewards but also social rewards like reputation and approval can promote the engagement of users, by analyzing the Steemit system, an example of DAOs. On the other hand, several studies also point out the poor decentralization or unfairness of Steemit~\cite{li2019incentivized, guidi2020graph, guidi2021analysis}. Another paper~\cite{gao2022true} focused on the NFT marketplaces to see if the token incentives can draw active participation of users in the DAO environment. Although they confirm the helpfulness of token incentives to induce user participation, our analysis results also cast doubt on that the token incentives alone can lead to healthy and robust DAO systems. In summary, there remain many challenges to what the proper incentives of DAOs are. 
\end{comment}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\noindent\textbf{AI-based intervention protocol with bubble-bursting fact-checks.} 
Fact-checking and moderation have been devised to encourage users to explore a wider range of viewpoints, transcend social media echo chambers, and ultimately decrease political and cultural polarization~\cite{wardle2017information,nekmat2020nudge}. 
In the context of DAOs, we have observed an unequal polarization among proposal voters, where whales exhibit homogeneous voting behavior among themselves, failing to represent the wider population. Experts have attributed this phenomenon to the lack of technical understanding of proposals of voters, leading them to follow the voting patterns of their trusted key opinion leaders. 
To address this polarization and echo chamber effect, an intervention protocol (in the form of a ML based recommender model) could be developed to enhance the credibility of information and prioritize fact-checking messages. Such a model would nudge DAO holders to learn more about proposals, thereby allow informed decision-making during voting rather than relying on the KOLs. This intervention protocol can allow diverse proposal content consumption during the soft proposal stage for both whales and grassroot voters.
%Additionally, this will enhance
%human agency in human-AI collaboration to enhance
%information integrity and warranted information trust, while preserving individual agency on social media platform

\noindent\textbf{Onchain proposal pipeline for autonomy \& ux.} 
%Nowadays, there are numerous onchain and offchain tools DAOs can use as part of their consensus pipeline. While useful tools like Snapshot provide an offchain, gasless, easy-to-use, and verifiable voting platform, the process of translating the consensus reached offchain to onchain actions is a bottleneck for both decentralization and autonomy as the onchain transactions are often manually crafted by a small group of people in most DAOs. 
%DAOs have access to a variety of onchain and offchain tools for their consensus pipeline. However,
Despite the benefits of offchain tools like Snapshot's gasless and verifiable voting platform, the manual translation of offchain consensus to onchain actions poses a bottleneck for decentralization and autonomy as the transactions are often manually crafted by a small group of people in most DAOs.
One solution to this could be moving the entire proposal pipeline onchain. While on-chain platforms encourage higher transparency and autonomy compared to Snapshot and Multisig, current on-chain systems of contracts are more difficult to deploy and maintain. Tools that allow DAO practitioners and users to have better user experience in deploying, maintaining, and interacting with fully on-chain DAO system of contracts can help achieve the best of both worlds. With features like stream payment and binding consensus being readily available onchain, this reduces the reliance on third-party services. In addition, in DAOs that suffer from long delays, being fully onchain opens up the possibility for any user to help issue the transaction to execute a proposal. 
Monetary incentives could also further incentivize users to execute DAO actions promptly. Of course, how to incentivize users in DAO would remain an open problem. 
Layer 2 solutions can help lower the gas cost for users, costing only a few cents to participate.

% Moreover, there exist many systems of smart contracts for DAOs that offer a higher degree of flexibility than Snapshot, with each having a different point of optimization (e.g., some for funding, and some for protocol governance). 

\noindent\textbf{Fully automated tracking tools for proposal transparency.} In examining third party dependent proposals, many proposals lack transparency during the execution period. This results in a handful of proposals having unknown status after passing the voting period. Reaching consensus alone is not enough to ensure autonomy. The resulting DAO actions must be easily verifiable by DAO members. At the moment, there are several tools employed by DAOs to publicly post and interpret DAOs action, such as Notion. However, there is a lack of adoption for fully automated tool to track proposal status from the start until after consensus is reached. In DAOs that rely heavily on employing third parties, fully automated tools that help track the progress of the task, end result, and payment are essential for DAO members to make an informed decision on compensation and future employments.

%The correlation result between gas cost and participation is inconclusive, with most DAOs showing insignificant correlation and some even significant positive correlation between them. This suggests that gas cost might unlikely be one of the main factors preventing individuals from participating in a DAO. However, we still believe that a cheap gas cost would help increase the participation of DAO users. From this perspective, alternative layer two chains, such as Arbitrium,
%\yujin{Citation? or examples} 
%could drastically lower the gas cost, encouraging users to more participate in DAO systems.

\begin{comment}
\begin{itemize}
    \item  What are the major parameters we examined?
    \item How can we say if it is a successful DAO?
    \item Number of metrics to quantifying successful DAO?
     \item Framework for characterize DAO
    \item Design implications 

\end{itemize}

\subsection{Predicting DAO Success}


%\yang{How can we say if this is a successful DAO? Number of metrics of quantifying successful DAO? Design implication for DAO platform? Framework for characterize DAO.}




\subsection{Metrics of quantifying DAO performance}



\subsection{Framework for characterizing DAO}





\subsection{Design implications for DAOs}

\end{comment}

==> arxiv_2024_S&P_DAO-Paper_final/section/Interview-Result.tex <==
\vspace{-2mm}
\section{Perceptions \& Practices of DAO Experts}
\vspace{-2mm}
\label{interview}
%briefly add P1, p2,   their invilvement of DAOs
Here, we report the result of our formative study. 

\noindent{\bf Expected level of decentralization.} Our interview findings indicate that there are varying perceptions and expectations for the level of decentralization 
%within DAOs. Our expert participants frequently discussed their perceptions of decentralization and indicated that it 
across different stages of DAO development. In particular, experts suggested that early-stage DAOs often require a certain level of centralization, as \textit{``at beginning to form it, it makes a lot of sense to be more centralized and move to a less centralized over time.''}
Experts also tended to differentiate decentralization in terms of technical and social aspects, noting that--\textit{``many facets of decentralization exist (perceptual, technical, legal) and that there are tensions between abstraction and practicality of Meloc V3 contracts.''} In discussing limitations to achieving expected levels of decentralization, experts pointed to certain types of DAOs (e.g., highly concentrated towards DeFi protocol DAO) that require centralization for effective operation. Some mentioned limitations in current factory contracts and called for the exploration of better utilization of smart contracts to increase decentralization. As P1, from Blockchain association and Polychain noted-\textit{``DAOs are pretty early. Many are just copying existing protocols. Maybe decentralization could be improved with newer contract or utilizing contracts.''} %These findings underscore the need for further research and the development of new approaches to decentralization in the context of DAOs.


\noindent{\bf Token-based economy lower decentralization.} We identified three metrics to evaluate decentralization, including token distribution, participation rate of token holders in voting/proposal, and members' geographies and regulatory risks.
Our experts compared the token holdings of the core team/founder to grassroots members. P3, who is involved in Aragon, Aave Hydra, DAOStar, noted that the token distribution remains largely unexplored in the context of decentralized governance-\textit{``If the founding team holds too many tokens, it disincentives others to contribute. For 'practical' decentralization, some other distribution is needed.''} 
%To measure decentralization, P7 suggested creating a knowledge base with a dictionary that includes price value Marketcap over time, which could be used to track the distribution of tokens and categorize them for exploring decentralization? of different categories of DAOs. 
%\korn{A bit confused by what the last sentence here meant.}
%Additionally, they noted that token-based governance is often inefficient and may hinder the achievement of true decentralization; for example, 
Similarly, P2, from his experience of LexDAO, SporusDAO, CaliDAO, onchain LLC, indicated token-based governance as inefficient, hindering the achievement of true decentralization; \textit{``we're coming to the conclusion that token-based governance, is ultimately not very effective because[...] if three or four whales out of 10,000 token holders have 51\% of the power. Can you really call it decentralized?''} 
Many emphasized the importance of assessing the participation rate of token holders during voting/proposals. 
%Our participants suggested that in addition to analyzing on-chain voting data, 
It is indicated as important to examine who is pitching the proposal and if they are from the core team. 
%P6 suggested contextualizing if the proposal meets the quorum with votes from whales. 
P6, previously worked in MakerDAO, and ConcenSys indicated that often proposals do not reach quorum without whale voters, and the proposal authors would chase down whale voters to lobby them to vote. Additionally, P8 noted that---\textit{``the reality is people don't like to participate in governance, [and] where you end up unfortunately, just speculating on the price value.''} Our experts pointed out the limitations of associating voting power with monetary value and suggested voting power to be proportional to contribution to DAOs. %Tokens that can be sold back to the governance are better than those that enable trading on secondary markets.
%Lastly, our experts mentioned the importance of considering DAO members' geography and related regulatory risks to effectively measure decentralization. However, they acknowledged that obtaining such information can be challenging due to the anonymous nature of blockchain-based applications.

\noindent{\bf Unclear concept of autonomy.}
%\yujin{How about this? ``Unclear concept of Autonomy''} 
Our interviews revealed a recurring theme of the absence of clear metrics for autonomy within DAOs. 
%Furthermore, our data suggest a lack of clear definitions and varying perceptions around autonomy. 
While many experts view autonomy as \textit{``less human intervention, more tool use,''} others noted that different levels of autonomy depend on the functions/types of DAOs. To avoid bias and excessive human interaction, some experts suggested creating \emph{``pods''} in DAOs for different operations, such as marketing or legal. As P5, working in Polywrap DAO, Llamadao noted, \textit{``we want to create different pods and each will have different people that are governing so one pod doesn't have too much power.''}
Some experts argued that relying on human intervention is necessary due to a lack of tooling, but emphasized the need to minimize dependence on external parties. Others defined autonomy in terms of the proposal and voting process, noting that--\textit{``if proposal/voting is happening within a machine, it's autonomous.''} Finally, a few experts defined autonomy in the context of, not being controlled by the US government, noting that---\textit{``I don't think it should honestly have to do with if people or machines can do quick execution. You can mean prolifically autonomous, is it not controlled by, say, US government.''} 
%These highlight 
%the need for a clearer definition and metrics for autonomy within DAOs, as well as 
%the importance of considering unique functions and types of DAOs in determining appropriate levels of autonomy.

\noindent{\bf Limitations of current tooling to enable autonomy.} Experts did not mention many solutions but instead suggested limitations in building autonomy in DAOs. Some of the limiting factors include execution time delays of DAO operations due to a lack of tooling, and proposals going into backlog due to quorum votes. P8, from DAOHQ noted that companies are attempting to improve user experience on the interface to make it easier for governance facilitators to support the process in a more automated, but there are not many options available. P7, involved in pleasr DAO, NounsDAO added that limitations around token holding and lack of interest in participating in governance often cause delays in the proposal process, since there are specific vote requirements to move the proposal forward. In this word---\textit{``Token distribution among a few or core members means a single point of failure, causing proposal delay.''}


\noindent{\bf Contextual factors making whales to vote in similar way.}
%Our network analysis of voting data identified that whale addresses tended to exhibit similar voting patterns among themselves, not necessarily being representative of the wider community. Through the interviews with key stakeholders, 
We identified several factors that might have contributed to similar voting patterns among whale voters. Some interviewees noted that the majority of whales belong to the managerial team leading to vote in a similar way. 
%These whales necessarily individuals who acquired tokens through participation in the DAO but rather through their association with the centralized managerial team. 
P5 noted---\textit{``so these whale,
%are kind of, not really whale in the sense that 
they started with a managerial, centralized team and so they are the largest token holders.''} Additionally, P5 added---\textit{``some of their communication happen through private channels like private discord, DMs or telegrams.''}, which may contribute to the similar voting patterns observed.  
Another factor contributing to this trend is people's trust in the voting of earlier whales. P8 noted that---\textit{``Honestly, for many proposals when earlier whales vote in a certain way, a lot of people just follow [..]many don't care to read through proposal. But they trust, whales know what they're doing.''} Peer pressure during the voting process was also mentioned as a factor that may lead individuals to vote in a similar way to the whales. 
%as they may not want to go against the consensus established by whales and impact their reputation in the community. 
P8 noted---\textit{``I didn't want to vote against the proposal, Just because, my reputation would be on the line or something.''} Overall, %the impression, 
\emph{whales running governance} is identified as a major limitation in DAOs.


\noindent{\bf Need for qualitative investigation alongside quantitative evidence.} Participants suggested that contextual factors should be incorporated including community sentiment from social channels, timing and the situation in which people join DAOs, additional financial metrics from existing exchanges, and the type of proposals being considered. 
%For example, P7 suggested looking at sentiment and stewardship in large ecosystems such as Bitcoin.
While higher proposal thresholds 
%were initially considered as indicative of less decentralization, DAO experts 
pointed out the trade-offs of protecting against spam or malicious proposals, 
%P8 noted that larger DAOs, such as Uniswap, set proposal thresholds based on token holdings to prevent spam and protect the system from malicious attacks. 
P9, from Gitcoin highlighted the practical implications of the threshold on the impact on DAO token value in terms of market capitalization.
%thus impacting the DAO's value.

==> arxiv_2024_S&P_DAO-Paper_final/section/Introduction.tex <==
\vspace{-2mm}
\section{Introduction}
\vspace{-2mm}
%Decentralized Autonomous Organizations (DAOs) are a novel form of organizational structure that utilizes smart contracts, which are computer programs encoded with specific rules and protocols, to govern their operations \cite{dwivedi2021legally}.For example, ConstitutionDAO where the rules and decision-making processes are encoded into a blockchain, allowing the terms of agreement between buyers and sellers to be directly written into lines of code. Members interact with the smart contracts through a user interface (UI) to participate in decision-making and access funds, and all actions are recorded on the Ethereum blockchain for immutability. UkraineDAO is another example which was built to launch a crowdfunding campaign to mint and sell non-fungible tokens (NFTs) of a Ukrainian flag in order to raise funds for Ukrainian civilians and the military~\cite{esteves2023potential, chaisse2022tokenised}.


%The governance of DAOs is a complex issue, as it is not yet clear to what degree they function in a truly decentralized ideal. Additionally, the influence of community involvement, decision-making authority, control measures, and the positioning of DAO members, which is reflected through proposals/voting, on the level of decentralization within a DAO, remains unclear~\cite{zachariadis2019governance}.Furthermore, the extent to which DAOs operates without undue external influence (potentially from corporate competitors or regulators, third parties) and the regulatory status of this organizational structure, are areas of ongoing research. The seemingly decentralized and autonomous nature (as the name of DAO implies) of DAOs makes them an exciting area for empirical research, as scholars seek to understand the implications of their unique structures and functions for governance, security and regulation. Quality governance, as a design objective for a DAO, aims to ensure effective and legitimate decision making~\cite{wang2019decentralized}. Conversely, regulators are primarily concerned with DAO of existing regulations and the determination of liability, which makes governance a focal point~\cite{mondaq}.

As of 2022, there have been over 4,000 decentralized autonomous organizations (DAOs) created with the goal to democratize the management structure for decentralized protocols and open-source projects~\cite{messari} utilizing smart contracts (i.e., computer programs encoded with specific rules) to govern their operations~\cite{dwivedi2021legally}. For example, in ConstitutionDAO, where the rules and decision-making processes are encoded into a blockchain, allowing the terms of agreement between buyers and sellers to be directly written into lines of code. UkraineDAO is another example which was built to launch a crowdfunding campaign to mint and sell non-fungible tokens (NFTs) of a Ukrainian flag to raise funds for civilian and military purposes~\cite{esteves2023potential,chaisse2022tokenised}. One of the key functions of a DAO is group decision-making, which is often conducted via a series of proposals where members vote with the DAO's governance tokens~\cite{coindesk}. The market value of such governance tokens typically signifies the relative influence of stakeholders within the DAO.
%In recent years, DAOs have also utilized non-fungible tokens (NFTs) to grant voting power and limit membership to those who confirm ownership of these tokens. 
%Decision-making in DAOs is often  conducted through a series of proposals on which members vote via the blockchain, with those holding more governance tokens having greater voting power.
Despite challenges faced by early DAOs, there are governance benefits to this structure, e.g., community-driven consensus, execution of predefined rules, transparency of the decision-making process~\cite{hassan2021decentralized, hackernoon}.
%The DAO structure provides governance benefits, including community-driven consensus, execution of predefined rules, and transparency of the decision-making process~\cite{hassan2021decentralized, hackernoon}.

However, the governance of DAOs is a complex issue; it is not yet clear to what degree they attain decentralization and autonomy, even though the name of DAO implies the two. Specifically, the influence of community involvement, decision-making authority, and positioning of DAO members in proposals and voting mechanisms on the level of decentralization remain unclear~\cite{zachariadis2019governance}. Furthermore, the extent to which DAOs operate without undue external influence (from corporate competitors, regulators, or third parties in general) in practice has not yet been explored. Therefore, systematic exploration is required in terms of procedural tedium\footnote{In the context of smart contract, while it aims to streamline protocol execution in the digital era, but still relies on tedious human involvement}, %\yang{need to explain this term}\tanusree{added a footnote}
 structural rigidity, community interaction, and voting manipulation through on-chain and off-chain data~\cite{zwitter2020decentralized, zwitter2020governance}. In this paper, we aim to discover how concretely  DAOs work in practice (focusing on decentralization and autonomy). We address the following research questions. 



\noindent \textbf{RQ1: What are the current perceptions \& practices of DAO participants in fulfilling DAOs' vision? 
%What is the current governance structure of these DAOs? and to what extent is a DAO fulfilling its vision?
} %\yang{these are two related but different questions. The results suggest that this RQ is more about DAO practitioners' perceptions of decentralization and autonomy} \tanusree{updated the question. yes, interview was to understand current practice (in context of Decentralization and autonomy) of DAO experts}
We conducted one-on-one interviews with 10 DAO participants and two focus groups (each with a dozen of DAO participants). %organizers and members. 
Our results reveal their nuanced perceptions and practices, e.g., \textit{``being decentralized is not the sole purpose''} and %their expectations for a certain level of centralization in early-stage DAOs. %They highlighted decentralization in terms of token distribution, and governance participation during voting/proposals while emphasizing the limitation of token-based economy leading to poor decentralization. Our findings indicated contextual factors, including 
why DAO participants often voted in a similar way was due to the influence of ``whales'' (i.e., those with a huge amount of governance tokens), trust in key opinion leaders, and peer pressure. 
%%Several contextual factors identified as contributing to poor decentralization, including majority whales belonging to the managerial team, many whales to trust the instinct of big whales or key opinion leader and peer pressure
% 
Our DAO participants varied in their definitions of DAO autonomy. While some viewed autonomy as \textit{``less human intervention, more tool use,''} others felt it is more about {\it without undue external influence}. %noted levels of autonomy depending on the functions and types of DAOs. 
We referred to the interview findings to establish metrics used in our follow-up analysis to explore RQ2 and RQ3.

%We then categorized DAOs into different types, such as De-Fi protocols, investments, public goods, and entertainment. We found that DAOs predominantly use predecessors' smart contracts or existing factory DAO contracts, such as DAOHaus, DAOstack, and Kleros, with some modifications to parameters such as the threshold of token holding for proposals and quorum votes. Finally, we defined a set of on-chain and off-chain metrics to help assess DAOs, including community interaction, voting patterns, voting power, arbitrary transaction execution, and execution delays. Majority of these factors were obtained from DAO experts' current practice. We used this initial set of metrics to conduct our empirical analysis to explore RQ2 and RQ3.


\noindent \textbf{RQ2: How decentralized is a DAO?} 
%\anote{This doesn't end up answered with a single scale, so maybe the question can be rephrased. It also doesn't end up with a clear baseline, i.e. what counts as "poor decentralization" from intro}
We investigate the decentralization degree of DAOs by analyzing on-chain and off-chain data.
%including proposal outcomes, proposers' information, token holdings, and organization categories. 
We find that token holdings have a significant positive correlation with proposal success in KrauseHouse, CompoundDAO, and dxDAO while for BitDAO, BanklessDAO, and AssangeDAO, there is no significant correlation, likely due to the presence of predefined whitelisted authors, community elected proposal authors, etc. CompoundDAO, AssangeDAO, Bankless, and Krausehouse exhibit high polarization in voting patterns indicating poor decentralization while Proof of Humanity (PoH), Meta Gamma Delta, and Moloch have a more equitable power distribution. Moreover, we find that members with more governance tokens tend to vote more actively, which deteriorates decentralization.   %using metrics such as Gini~\cite{dorfman1979formula} and Nakamoto coefficient~\cite{earn}%yujin{Removed this cause the above sentence is not for the analysis using the two metrics.}
Finally, the decentralization level has been gradually aggravated in CompoundDAO, BitDAO, and BanklessDAO, which have governance based on token capital, while it has improved over time in the one-person-one-vote DAO, PoH. 
%Additionally, we discuss the contextual factors of decentralization, including the need for decentralization to be established at both the infrastructural and governance levels, and the relationship between decentralization level and gas fee to vote. Our findings indicate that there may be other factors that determine the decentralization level of a DAO voting system.

%Overall, this research provides insight into the complexities of achieving decentralization in DAOs and highlights the need for further examination of the various factors that may impact the decentralization level of a DAO voting system.




\noindent\textbf{
%RQ3: How well crafted are DAO smart contracts?%
RQ3: How autonomous is a DAO?
}
%\yang{missing the connection between autonomy and how well crafted smart contracts are. and what do we mean by well crafted?} \tanusree{updated the RQ. well crafted means- smart contract that can perform "without undue external influence" I think "How autonomous a DAO? would be more suitable" since in our case , we considered both-- (1) less human, more tool; (2) without undue external influence for analysis}
%To answer this question, we evaluated 10 DAOs to understand their level of autonomy and the degree to which they operate without undue external influence, potentially from corporate competitors or regulators.
Based on inputs from our interviews and focus groups, we considered two aspects of DAO autonomy: (1) less human intervention, more tool usage; and (2) without undue external influence.
% 
%To answer this question, we evaluated 10 DAOs for their capability to execute arbitrary transactions without unnecessary external intervention, number of proposals relying on third parties after execution, number of proposals canceled after the voting period ends and the execution delay. 
%These metrics explore how the current DAOs' infrastructures support autonomy and to what extent autonomy is respected in practice. 
Our analysis revealed variations among DAOs to achieve arbitrary transaction execution, with on-chain proposal submission being the most autonomous via code modules. %\yang{by autonomous, you meant tool usage rather than human intervention?} \tanusree{yes, here "tool" means the smart contract protocol, vote/proposal offchain modules, etc}. 
We also observed most DAOs require 3rd-party services to operate. 
%with the most common case being employment for future services. 
%Our data on the number of proposals canceled after voting ends suggests that DAOs tend to follow proposal binding ideology, even if it is not guaranteed programmatically. 
%Furthermore, the existence of a large number of DAO proposals with unknown status suggests a need for proposal transparency tools.  
%We also found that execution delay varies from 4 hours to 6 days.
%There was no statistically significant correlation between the gas price in ETH and the proposal execution delay.
%, with high gas prices impacting smaller treasury DAOs' delay. Overall, our study provides insights into the extent to which autonomy is respected in practice
%We also found that the execution time delay varies from 4 hours up to 6 days for on-chain DAOs, with high average gas prices being a possible factor impacting the length of delay, particularly for DAOs with smaller treasuries. 
%Overall, our research sheds light on the complexities of achieving autonomy in DAOs and  the importance of strategies to minimize the risk of third-party reliance.
%\yang{need to summarize the main contributions}\tanusree{done}

\noindent{\bf Main contributions.} Our work makes the following contributions: 
(1) We offer novel insights into the perceptions and practices regarding the degree of decentralization and autonomy in fulfilling the visions of DAOs by interviewing DAO participants.
(2) Through our empirical analysis of on-chain and off-chain voting/proposal systems, as well as assessments of corresponding smart contracts, we shed light on the level of decentralization and autonomy in DAOs using key metrics, some of which we learned from the DAO participant interviews. 
(3) Based on our empirical results, we discuss design implications for governance models of DAOs and DAO tooling such as DAO proposal transparency tools. %incentivizing mechanisms to increase engagement among DAO holders.

%\yang{human? external?} \korn{updated} 
\begin{comment}
The remainder of this article is organized as follows: In Section \ref{related_work}, we provide an overview of the history and evolution of DAOs, their governance structures, incentives and participation, and the challenges faced by 
%\yang{faced by?} \korn{Updated} 
DAOs. In Section \ref{research_approach}, we present the method of this study and the metadata for the empirical analysis. Section~\ref{section4} summarizes the findings of our analysis of 10 DAOs and their current landscape, including macro level insights. In Section~\ref{section5}, we present our empirical observations and the case studies of the 10 DAOs that we have conducted to evaluate the effectiveness of DAO governance protocols for decentralization. In Section~\ref{section6}, we present our findings on the autonomy level of the DAOs. Finally, in Section~\ref{section7}, we map the explicit knowledge of DAO experts to the explicit knowledge of DAO platforms that we have captured based on our empirical studies. We provide a set of DAO design implications and suggestions for future research.
\end{comment}

==> arxiv_2024_S&P_DAO-Paper_final/section/Macro-Result.tex <==
\vspace{-2mm}\section{Summary of 10 DAOs}
\label{section4}
\vspace{-2mm}

%We analyzed different categories of DAOs (e.g. DeFi, investment, entertainment, social, etc.) which were formed between 2019 and 2022.  
%with 10 specific DAO projects  
In this paper, we selected 10 DAOs, which were formed between 2019 and 2022, prioritizing diverse categories (e.g., investment, defi, video, social, etc), popularity, and market capitalization. To add diversity for governance design, we, in particular, considered four DAOs, created with popular DAO factory contracts, including Governance Bravo 
DAOhaus, Kleros, and DAOStack, in the governance structure.
Table~\ref{tab1:macro} presents the key parameters of the 10 DAO projects, including the treasury size, number of DAO holders, active voters, total votes, participation rate in proposals, number of proposals, number of proposal creators, quorum voting, and proposal threshold (more details in Appendix~\ref{10_dao}). 
%Despite a significant growth in market capitalization, crucial information is missing from various resources for all existing DAO projects, indicating limited transparency and highlighting the need for a comprehensive service that can provide more detailed analytics for these projects.


 \begin{table*}[]
 \scriptsize
\begin{tabular}{llllllllllll}
\hline
DAO               & Category                                               & Treasury & \#Holders & \#Active & \begin{tabular}[c]{@{}l@{}}Avg \\ votes\end{tabular} & Participation \% & \# proposal & \#votes & \#Creator & \begin{tabular}[c]{@{}l@{}}Proposal \\ Threshold\end{tabular} & Quorum\\
\hline
CompoundDAO       & Protocol                                               & 90.7M    & 205.9k    & 4.1k     & 78                                                           & 1.80\%           & 137         & 12750   & 48        & \begin{tabular}[c]{@{}l@{}}25000\\ COMP\end{tabular}          & 400,000                                                \\

BitDAO            & Investment                                             & 1.6B     & 20.4k     & 320      & 53                                                           & 1.30\%           & 19          & 1347    & 14        & \begin{tabular}[c]{@{}l@{}}200,000 \\ BIT\end{tabular}        & 100,000,000                                                                            \\
AssangeDAO        & Social                                                 & 242.9k   & 6.3k      & 1.1k     & 298                                                          & 12.30\%          & 11          & 3576    & 2         & \begin{tabular}[c]{@{}l@{}}1,000\\  JUSTICE\end{tabular}      & 867,576,97                                                                             \\
Proof of Humanity & Social                                                 & 801.7k   & 35.2k     & 3.1k     & 153                                                          & 8.80\%           & 104         & 16557   & 25        & 0 VOTE                                                        & NA                                                                                     \\
Bankless DAO      & Web3 fund                                              & 1.6M     & 5.9k      & 3,375    & 344                                                          & 43\%             & 51          & 18272   & 7         & 0 BANK                                                        & NA                                                                                    \\
KrauseHouse       & Sports                                                 & 1.2M     & 1.8k      & 595      & 32                                                           & 30\%             & 131         & 4,484   & 5         & \begin{tabular}[c]{@{}l@{}}1,000 \\ KRAUSE\end{tabular}       & 0                                                                                      \\
LivePeer          & Video                                                  & 0        &   NA        &    NA      &           NA                                                   &     NA             & 7           & 600     & 7         & 0 LPT                                                         & 1/3*27,004,976                                                                         \\
MetaGammaDelta    & Social                                                 & 29.7k    &  NA         & 49       & 2                                                            & 29.40\%          & 79          & 132     & 30        & 1 DAI                                                         & 0                                                                                      \\
MolochDAO         & \begin{tabular}[c]{@{}l@{}}Public \\ Good\end{tabular} & 0.1      & NA          & 60       & 4                                                            & 50.80\%          & 32          & 83      & 29        & 1 WETH                                                        & 0                                                                                      \\
dxDAO             & Protocol                                               & 81M      & 1.4k      & 232      & 2                                                            & 5.80\%           & 864         & 3161    & 160       & 0 rep                                                         & \begin{tabular}[c]{@{}l@{}}0 if boosted \\ else 50 \% REP\\  token supply\end{tabular}\\
\hline
\end{tabular}
\caption{DAO Projects Summary in terms of macro information\vspace{-2mm}}
\label{tab1:macro}
\end{table*}


Among 10 DAO projects, five perform off-chain voting (BitDAO, AssangeDAO, Bankless, KrauseHouse, and Proof of Humanity), while the rest perform on-chain. Gnosis Safe~\cite{gnosis} Snapshot platform is often used for off-chain voting aggregation for its user-friendly interface. However, it is not implemented in blockchain and requires further action from the operation team through multi-sig~\cite{daohaus}.
Across 10 different DAOs, the requirements vary significantly. For instance, BitDAO and CompoundDAO only allow whitelisted addresses to propose, and proposal submissions require a specific amount of tokens above a certain threshold. However, the threshold is often too high for grassroots users\footnote{The ``grassroot users'' cluster represents addresses with token holding that is less than the whale address token threshold.} to propose without delegation from others, resulting in industry entities or large token holders submitting most proposals. AssangeDAO, BanklessDAO, and KrauseHouse only permit authors verified on snapshot to propose. 
%In Proof of Humanity, the proposal requirement changed from allowing anyone to propose to only committee or elected members. 
In Livepeer, anyone with a sufficient amount of staked\footnote{Staked governance tokens are locked for a period of time. Those that stake their tokens often bear certain protocol risks.} governance tokens can propose, while in Meta Gamma Delta and MolochDAO, proposals require sponsorship\footnote{Sponsoring proposals in Moloch and Meta Gamma Delta DAO is an act in which a DAO shareholder moves the proposal into the voting pipeline.} from a member. Lastly, dxDAO has the most flexible proposal requirement, allowing anyone to propose. Each DAO also has a specific quorum voting strategy for accepting proposals, with CompoundDAO requiring 400,000 COMP, BitDAO requiring 100,000,000 BIT, AssangeDAO requiring 867,576,975 JUSTICE tokens, etc.











==> arxiv_2024_S&P_DAO-Paper_final/section/Method.tex <==
\vspace{-2mm}
\section{Methodology}
\label{research_approach}
\vspace{-2mm}
% \tanusree{elaborates on how we have mapped the knowledge of DAO platforms that we have captured based on an extensive off-chain and on-chain data. explains our empirical observations in the context of 5 real-world case studies (of different categories) that have been conducted to evaluate the effectiveness and usefulness of the decision model in addressing the DAO Platform a) Discovery/creation criteria, b) Future success of DAO governance structure. c) metrics of DAOs. 
% study of wikipedia, ed chi, how wikipedia governance work, editing policy
% https://www.cc.gatech.edu/people/munmun-dechoudhury
% }
% In our research method, there are different approaches, such as, observation, social network data, etc.), inference techniques (taxonomy, protocol analysis, statistics, etc.), units of analysis (individuals, groups, process, etc.),and so forth \cite{}.

To have an in-depth understanding of various DAOs, we adopt a mixed-methods approach, iteratively blending quantitative and qualitative analyses which involve multiple sources of data, including off-chain and on-chain data. 




\subsection{Empirical Analysis}
We conduct an empirical analysis of DAOs at both macro and meso levels.
%focusing on their contribution to the crypto market, growth patterns over time, descriptive statistical properties of the DAO market, network structure of DAO holders' voting behavior, factors influencing decentralization and autonomy in DAOs. 
Our analysis begins with an exploration of on-chain and off-chain voting data, specifically measuring the frequency of new addresses and users engaging in DAOs, as well as the evolution of DAO growth, funding patterns, treasury amount, and categories of DAOs. We then focus on the governance structure of each DAO, using descriptive statistics at the macro level to identify community members involved in DAO activities such as voting and proposing, different governance mechanisms, including proposal threshold, eligibility of proposal, quorum voting, etc. 

We then use these entry points to conduct in-depth quantitative analyses, expanding upon the existing theoretical framework for investigating both on-chain and off-chain voting and proposal data.
At the meso level, we use different methods of network analysis, economic and information theory (e.g., gini, nakamoto co-efficient, entropy) presented in the literature to investigate how different factors, such as voting power, similarities and differences among DAO holders, and token holdings, are assembled to identify the positionality of DAO holders within the network, and how this influences the decentralization. We also examined the underlying smart contract to assess to which capacity DAOs operate with less human intervention and without undue external influence, potentially from corporate competitors or regulators.
We provide additional details about specific methods, and analysis results in Sections~\ref{metric-method}, \ref{section5}, and \ref{section6}. %, with analyses conducted iteratively. 
%often moving back and forth from one level to another as insights from one informed new questions to investigate at another. 
While we did not extensively explore the potential influence of online forum interactions on on-chain and off-chain governance decision-making in this empirical analysis, we added narratives of different soft proposal discussions where appropriate and provided suggestions for future research to combine these two information spaces in the analysis. 
We provide a summary along with the current limitations of the metrics and methods used to explore \textbf{RQ2} and \textbf{RQ3} in Appendix~\ref{metric-method}.

%

\subsection{Data Collection}
We collected both off-chain data including DAO proposals, voting, token, and treasury smart contracts, as well as off/on-chain voting smart contract modules. %Furthermore, blockchains store massive amounts of heterogeneous data that grows over time. 
For DAOs having readily available source code, we turned to Etherscan~\cite{Etherscan} while it has become the de-facto source for Ethereum blockchain exploration. It offers a useful feature called \emph{``verified''} contracts, where contract writers can publish source code associated with blockchain contracts. Etherscan then independently verifies that the compiled source code produces exactly the bytecode available at a given address. 
%Etherscan then makes the verified source available to the public. 
We scraped contracts as of November 2022. 
We then checked contracts with corresponding GitHub sources to determine the correct complied version for our analysis. For MolochDAO, Meta Gamma Delta, and dxDAO, we aggregated factory contracts from DAOhaus and DAOstack.

Focusing on the network that DAOs are built upon, we searched for voting and proposal information sources on the blockchain (on-chain DAO) and the corresponding voting platform (i.e., snapshot for off-chain DAOs). If necessary, we directly access records (blocks) using a unique identifier (e.g. block ID, transaction, wallet, or contract address). As a result, we build scripts and data pipeline/techniques for data extraction in order to conduct an analysis effectively without having to sequentially walk through all the blockchain or offchain platform data. Table~\ref{tab:metadata} lists three main forms of data including smart contracts, on/off-chain proposals, and on/off-chain voting. We collected the data in a comma-separated value.
%and json files per the analysis needs. 



\begin{table}[]
\scriptsize
\begin{tabular}{lll}
\hline
%\rowcolor[HTML]{FFFFFF} 
Smart Contract Data & DAO Proposal Data                & Data Voting Data                                     \\
\hline
%\rowcolor[HTML]{FFFFFF} 
\begin{tabular}[c]{@{}l@{}} \\ Compound Bravo\\ DAOhaus\\ DAOstack\end{tabular} & \begin{tabular}[c]{@{}l@{}}Proposal Author\\ Proposal Title\\ Proposal description\\ Proposal Timestamp\\ Proposal start/end Block\\ Author Token Wieght\\ Proposal Signatures\\ Proposal Outcome \\ Proposal State \\ Proposal Gas Cost \\ Execution Time delay\\ intendedExecutionTime\end{tabular} & \begin{tabular}[c]{@{}l@{}}Voter Address \\ Voter Organization\\ Voter Token Weight\\ Voter Average Token Weight\\ Voter Name if available\\ Voting Pattern (1, -1, 0)\\ Voting txHash\\ Voting Gas Cost(ETH)\\ Voting Gas Cost(USDT)\\ Voter Timestamp\end{tabular} \\

\hline
\end{tabular}
\caption{List of Metadata collected for off/on chain DAOs \vspace{-2mm}}
\label{tab:metadata}
\end{table}

\vspace{-2mm}
\subsection{Formative Studies}
\vspace{-2mm}

Our formative study encompasses both individual and group sessions, comprising eight individual interviews, one group session with ten experts representing diverse DAO communities, and a break-out session with more than 10 experts in DAO governance (demographics details in Appendix~\ref{demo-formative}). The purpose of this study was to gain insights into the existing DAO governance practices. We further aim to identify and establish a set of metrics to assess the effectiveness of governance structures, as viewed through the perspective of experts, who predominantly consisted of DAO founders and leaders. 
%In particular, we focused on exploring our first research question \textit{``What is the current governance structure of these DAOs? and to what extent is a DAO fulfilling its vision?''}. 
To this end, the study sought to explore on-chain and off-chain metrics (e.g., proposal threshold, active voters) that DAO experts perceived as contributing to the evaluation of DAOs in practice and how these metrics were defined and quantified by experts.

%and any additional metrics that DAO experts think can play essential roles to assess DAOs and how do they define and quantify those metrics. 

We began by introducing ourselves and outlining our project's objective of gaining insight into how DAOs operate in practice. We then briefly presented our initial ideas on metrics for both decentralization and autonomy, such as voting patterns, proposal success, execution delay, 3rd party reliance, etc, to obtain feedback from the DAO experts. We encouraged participants to share their experiences with DAO governance and ideas for additional metrics. We also inquired about the primary goals of the specific DAOs
%we asked them to reflect on their governance practices. 
that they are involved with. We then asked whether there have been any significant changes to their governance policies. 
%such as modifications to voting mechanisms and membership structures, or the workflow of decision-making, such as the voting platform or who gets to participate in voting.
%We posed questions such as \textit{``What's the primary goal of the DAO you are working on? Are there significant changes to the governance policies? Is there a way to dispute the decision? Is the proposal outcome binding?''} 
We also probed their views on the level of decentralization and autonomy in their DAOs.
%as well as how legal issues are handled within the DAOs they are involved in. 
Finally, we asked for their desired tools to aid in governance and the set of features they would recommend for governing and evaluating DAOs.


\iffalse
\subsection{Current Perception \& Practice of DAO Experts}
%\tanusree{will add interview findings here}

%\subsubsection{Perception of Decentralization \& Autonomy}
\label{interview}
In this section, we report the result of our formative study. \yujin{We don't need to present some profiles of interviewees? If this is combined with discussion, I don't think we need this.} \tanusree{yes, discussing their profile can reveal their identify. however, I will add a table in appendix including their generalized demographics and areas of expertise in DAOs}

{\bf Expected Level of Decentralization.} Our interview findings indicate that there are varying perceptions and expectations surrounding the level of decentralization within DAOs. Our expert participants frequently discussed their perceptions of decentralization and indicated that it differs across different stages of DAO development. In particular, experts suggested that early-stage DAOs often require a certain level of centralization, as \textit{``oftentimes when people are beginning to forming it, it makes a lot of sense to be more centralized at first and move to a less centralized state over time.''}

Experts also tended to differentiate decentralization in terms of technical and social aspects, noting that---\textit{``many faces of decentralization exist (perceptual, technical, legal) and that there may be tensions between the abstraction and practicality of Meloc V3 contracts.''} In discussing limitations to achieving expected levels of decentralization, experts pointed to certain types of DAOs (e.g., highly concentrated towards De-Fi Protocol DAO)
%\yujin{We need to mention the types of DAOs?} 
that require centralization for effective operation. Additionally, they noted that token-based governance is often inefficient and may hinder the achievement of true decentralization; for example, P2 noted \textit{``I think we're starting to come to the conclusion that token-based governance, especially, is ultimately not very effective because especially if the tokens are transferable if three or four whales out of 10,000 token holders have 51\% of the power. Can you really call it decentralized?''} Finally, some experts mentioned limitations in the current factory contracts and templates used to start off DAOs, and called for the exploration of newer contract architectures to increase decentralization. As P1 noted---\textit{``One thing to keep in mind: DAOs are pretty early. Many are just copying existing protocols. Maybe decentralization could be improved with newer contract architectures.''} These findings underscore the need for further research and the development of new approaches to decentralization in the context of DAOs.


{\bf Unclear Concept of Autonomy.}
%\yujin{How about this? ``Unclear concept of Autonomy''} 
Our interviews revealed a recurring theme of the absence of clear metrics for autonomy within DAOs. Furthermore, our data suggest a lack of clear definitions and varying perceptions around autonomy. While many experts view autonomy as---\textit{``less human intervention, more tool use,''} others noted that different levels of autonomy depend on the functions and types of the DAOs. To avoid bias and excessive human interaction, some experts suggested creating \emph{``pods''} within DAOs for different aspects of operation, such as marketing or legal governance. As P5 noted, \textit{``we want to create different pods like a marketing pod, the legal pod and so on. And then each of these will have different people that are governing so that one pod doesn't have too much power.''}

Some experts argued that relying on manual human intervention in DAOs is sometimes necessary due to a lack of tooling around certain functions, but emphasized the need to minimize dependence on external parties. Others defined autonomy in terms of the proposal and voting process, noting that---\textit{``if proposal/voting is happening within a machine, it's autonomous.''} Finally, a few experts defined autonomy in the context of organizations not being controlled by the US government, noting that---\textit{``I don't think it should honestly have to do with whether people or machines can do quick execution or not. You can mean prolifically autonomous, is it not controlled by say the US government, which means it is not controlled by any single entity.''} These findings highlight the need for a clearer definition and metrics for autonomy within DAOs, as well as the importance of considering the unique functions and types of each DAO in determining appropriate levels of autonomy.

%\subsubsection{Potential Assessment Metrics}

%DAO experts in our interview mentioned several potential metrics in assessing decentralization in mainly three different context, including, How well token is dispersed/distributed, participation rate among token holders during voting/proposals, decentralization in terms of members' geographics and related regulatory risks. 
%In context of token distribution, experts suggested to compare token holding of core team/DAO founder to other members (grassroot). To illustrate current limitation, P3 noted that token distribution is still unepxlored in decentralized governance mission and noted that-\textit{``Power of the founding team is a problem, If the founding team holds too much tokens, it disincentive others to contribute. For “practical” decentralization, some other token distribution is needed''} Some also suggested to create a knowledge base with 
%dictionary, including price value Marketcap overtime to measure decentralization. More specifically, P7 noted- \textit{``knowledge base with low, high, that sort of LCD things, you can see transactions of holders, and see the distribution, proposals, community, etc to categorize those for decentralization.''}
%Majority participants mentioned about holders' engagement during voting / proposal. In addition to on-chain voting data, they suggested to look behind the scene to identify who is pitching the proposal and if they are from core team. They also suggested to contextualize if the proposal meet quorum with the votes from whale address. P6 noted by illustrating current experience -\textit{`` Do they reach quorum without whale voters. oftentimes they don't, so behind the scenes, the proposal maker chase down Whale voters lobby to them to vote.''} To add more context, P8 mentioned that the reality of not many people being interested in governance than the speculative profit-\textit{``the reality is people don't like to participate in governance, blockchain space still like a lot of speculators[...]where you end up unfortunately, just speculating on the price value of something.''} Lastly they mentioned about the limitation of \empg{associating voting power with monetary value}. To illustrate that, P3 noted -\textit{``Voting power should be proportional to contribution to the project and need fixing for token distribution to founding team. tokens that can sell back to the governance is better than those enable trading on secondary market''} Finally, they mentioned about adding more contextual information such as DAO members' geography and related regulatory risks to effectively measure decentralization, however, much of these information are not feasible to achieve due to the anonymous nature of blockchain based application. 

{\bf Limitation of Token-based Economy.} We identified three aspects from experts to evaluate decentralization, including, token distribution, the participation rate among token holders during voting/proposals, and members' geographies and regulatory risks.
Regarding token dispersion, our experts suggested comparing the token holding of the core team or DAO founder to that of grassroots members. P3 noted that the distribution of tokens remains largely unexplored in the context of decentralized governance. Furthermore, P3 noted---\textit{``If the founding team holds too many tokens, it disincentives others to contribute. For 'practical' decentralization, some other token distribution is needed.''} To measure decentralization, P7 suggested creating a knowledge base with a dictionary that includes price value Marketcap over time, which could be used to track the distribution of tokens and categorize them for exploring decentralization? of different categories of DAOs. 
%\korn{A bit confused by what the last sentence here meant.}


Most of our interviewees emphasized the importance of assessing the participation rate of token holders during voting/proposals. Our participants suggested that in addition to analyzing on-chain voting data, it is important to examine who is pitching the proposal and if they are from the core team. P6 suggested contextualizing if the proposal meets the quorum with votes from whales. P6 noted that often proposals do not reach quorum without whale voters, and the proposal maker would chase down whale voters to lobby them to vote. Additionally, P8 noted that the reality is that not many people are interested in governance compared to speculative profit. In his word---\textit{``the reality is people don't like to participate in governance, [and] where you end up unfortunately, just speculating on the price value of something.''} Additionally, our experts pointed out the limitations of associating voting power with monetary value and suggested that voting power should be proportional to contribution to the project. Tokens that can be sold back to the governance are better than those that enable trading on secondary markets.
Lastly, our experts mentioned the importance of considering DAO members' geography and related regulatory risks to effectively measure decentralization. However, they acknowledged that obtaining such information can be challenging due to the anonymous nature of blockchain-based applications.

{\bf Limitation of Current Tooling to Enable Autonomy.} Regarding the current autonomy assessment strategies, experts did not mention many solutions but instead suggested limitations in building autonomy in DAOs. Some of the limiting factors include execution time delays of DAO operations due to lack of tooling, and quorum votes as a limiting factor for proposals to go into backlog. P8 noted that companies are attempting to improve user experience on the interface to make it easier for governance facilitators or managers to support the process in a more automated and trusted way, but there are not many options available. P7 added that limitations around token holding by broader holders and lack of interest in participating in governance often cause delays in the proposal process, since there are specific vote requirements to move the proposal forward. In this word---\textit{``Token distribution among a few or core members means a single point of failure, causing proposal delay.''}


{\bf Contextual Factors Making Whales to Vote in Similar Way.}
Our network analysis of voting data identified that whale addresses tended to exhibit similar voting patterns among themselves, not necessarily being representative of the wider community. Through the interviews with key stakeholders, we identified several factors that might have contributed to this trend. For example, some interviewees noted that the majority of whales belong to the managerial team, which leads to them voting in a similar way. These whales are not necessarily individuals who acquired tokens through participation in the DAO but rather through their association with the centralized managerial team. P5 noted---\textit{``so these whale are kind of, not really whale in the sense that they started with a managerial, centralized team. And so they are the largest token holders.''} Additionally, P5 added---\textit{``some of these communication might be through private channels like private discord, DMs or telegrams.''} which may contribute to the similar voting patterns observed.  
Another factor contributing to this trend is people's trust in the earlier voting patterns of whales.
P8 noted that---\textit{``Honestly, for many proposals I feel like when the earlier whales vote in a certain way, a lot of people just follow, just follower pattern, [..]I mean, many don't care to read through the proposal, think through it. But they trust, these whales know what they're doing.''} Peer pressure during the voting process was also mentioned as a factor that may lead individuals to vote in a similar way to the whales, as they may not want to go against the consensus established by whales and impact their reputation in the community. P8 noted---\textit{`` I didn't want to vote against the proposal, Just because, my reputation would be on the line or something.''} Overall, the impression, \empg{whales running governance} is identified as a major limitation in DAOs.


{\bf Need for Qualitative Investigation Alongside Quantitative Evidence.} Majority of the participants suggested 
incorporating contextual factors into the quantitative empirical analysis. Key contextual factors include community sentiment from social channels, the timing and situation in which people join a DAO, additional financial metrics from existing exchanges, and the type of proposals being considered. For instance, P7 suggested to---\textit{``take a look at sentiment. And something else is stewards, especially in like the big ecosystems like Bitcoin, who's active on the discourse?''} While higher proposal thresholds were considered indicative of less decentralization from a quantitative perspective, DAO experts pointed out interesting trade-offs for having higher thresholds, such as protecting against bad, spam, or malicious proposals. P8 noted---\textit{``often see larger DAO, uniswap, putting a threshold to propose and it's tied to the token most of the time, how much you're either delegated or that you personally hold. they wanted to keep a threshold to avoid spam and protect the system from malicious attacks.''} 
P9 highlighted the practical implications of proposal thresholds, such as their impact on the value of DAO tokens in terms of market capitalization. P9 noted---\textit{``token Holdings is related to how much market value dao will have in future, because if they do have threshold for people to make a proposal, then they will have to have this token amount from governance token and that market price can increase when people are buying this token, do you think that that could also have some impact of dials to have a certain threshold.''}


\fi















\begin{comment}
\paragraph{Capability of Arbitrary Transaction Execution}
%\subparagraph{Summary}
Nowadays, there exists multiple methods in translating the DAO's consensus into onchain action \yang{an on-chain record?}. While the governance process can be done entirely onchain to ensure bindingness of the consensus with minimal human intervention in executing the DAO action, many existing DAOs choose to trade autonomy for simpler methods. We explore such methods for the 10 DAOs from the perspective of autonomy by investigating how and to what degree individuals can influence this process in their favor.
\paragraph{Limitations}
Despite the process being highly manual in retrieving the source code and analyzing methods DAOs use to issue onchain transactions, the results are applicable to many DAOs as 
DAOs tend to use existing factory contracts and pre-made methods in issuing onchain transactions.

\paragraph{Third-Party Dependent Proposals After Execution}
%\subparagraph{Summary}
Third-party dependent proposals refer to proposals that rely on third-party actions to achieve their goals.  
Translating the consensus into onchain proposal execution is only half of the picture of the proposal execution process as some proposals can not be completed onchain. Some examples of such proposals could be hiring someone to host an offline event or hiring someone to write a smart contract. In this study, third-party actions refer to any action not originated from the DAO proposal pipeline. 
%Third-party dependent proposals refers to proposals that rely on third-party action to achieve its goal. 
Execution refers to the timestamp for onchain conclusion of the proposal. In the case of hiring a third party to do some work, third party action refers to the work delivered by the third-party and the point of execution refers to onchain record for employment, usually comes in the form of salary payment. While interaction with third-parties is inevitable for most DAOs, the number of third-party dependent proposals after execution can serve as a proxy for the number of occurrences the DAO autonomy \yang{I think we need to revisit the definition of autonomy esp. given Andrew's earlier comment} is being threatened. Generally, a smaller number of such proposals means a higher level of autonomy. In this section, we quantify the occurrences of such proposals in each DAO and identify strategies DAOs currently employ to mitigate the autonomy risk while still benefiting from third-party services.
\paragraph{Limitations}
In identifying whether a transaction is dependent on third-party after execution, it can be difficult for us (external researchers) to objectively make such a determination. Our proposed criteria of categorization may not be applicable to every DAO due to the diversity in the DAO proposal content. The process is also labour intensive and can be error-prone as it requires manually going through the proposal content, community discussions, and onchain transactions to understand the context of the transaction.
\paragraph{Canceled Proposals After Voting Ends}
%\subparagraph{Summary}
One way a DAO autonomy could be hampered is through proposal censorship. Proposal censorship refers to the act of not carrying out the proposal action after the community consensus has been reached. Having a small group of people translating consensus into DAO's onchain action can be viewed as an autonomy bottleneck as that group of people have to power to censor or manipulate the community consensus result. We empirically quantify the event of proposal censorship in the 10 DAO using a combination of onchain transaction data and offchain community discussion data.
\paragraph{Limitations}
For DAOs that have their governance done onchain, calculating the number of canceled proposals after voting ends can often be done through crawling emitted smart contract events. The process for offchain DAOs, however, is much more manual as it requires a mapping between offchain proposal data and onchain transactions. Due to the vast number of proposals, not all proposals can be determined if they have been executed or canceled. This highlights the lack of proposal transparency tools in the field.
\paragraph{Execution Time Delay}
%\subparagraph{Summary}
Part of autonomy includes the DAO's capability to promptly convert consensus into onchain action. Some DAOs rely on a small group of people to issue a transaction while some others allow anyone to issue a predetermined proposal transaction after the consensus has been reached. We collected the execution time delay data, which is the difference between actual execution time and the intended execution time, of the 5 onchain DAOs. The average execution time delay is compared across DAOs. For each DAO, we conducted a correlation analysis between network congestion and execution time delay to explore the relationship between the two variables.
\paragraph{Limitations}
Limitations for execution time delay analysis are similar to canceled proposals after voting ends analysis, where proposal timeline data can be fetched through emitted smart contract events for onchain DAOs and much more manual for offchain DAOs.
%\yang{it'd be nice to have a table of the metadata}
\end{comment}


% \begin{table}[]
% \begin{center}
% \begin{tabular}{|l |l|l} 
%  \hline
% Type of Data & Name of Data & Details\\
%  \hline
%  Overall Macro Data &\\
%  DAO Proposal Data &\\
%  Data Voting Data &\\
%  Smart Contract Data&\\
%  \hline
% \end{tabular}
% \caption{Data Collection with details}
% \end{center}
% \label{tab:metadata}
% \end{table}



% \subsubsection{Twitter Data}
% Data was obtained from a collection related to the BitDAO, which consists of tweets posted between April, 2021 to Feb, 2022. We collected the data using the Twitter Streaming API, tracking various keyword terms related to the BitDAO in real-time. We also collected data from Twitter BitDAO page via Twitter streaming API. We then scoped this data to tweets that contained BitDAO Twitter identified as English (denoted by the language code “EN” in the tweet metadata). The rationale for collecting English tweets was based upon our interest in how information operations in BitDAO designed for western audiences are taking shape in online spaces and how those engagement influence the BitDAO governance structure, voting and proposal for funding assignments. We acknowledge that conversations around these same topics in other languages would likely look different. Our dataset consisted 215 original tweets from BitDAO twitter page and 179 by searching with "BitDAO" terms, totaling 394 tweets, retweets, authored by X distinct accounts. 

%\subsection{Data Analysis}


% \subsection{Expert Interviews}
% \textbf{could we do some expert interviews of the DAOs we are doing case studies?}
% \yang{that'd be great}

% \begin{table}[]
% \begin{center}
% \begin{tabular}{|l |} 
%  \hline
% \textbf{RQ1}: What is the current governance\\
% structure of DAOs?\\ [0.5ex] 
% \hline
% \textbf{RQ2}: What could be applied as benchmarks\\
% to evaluate DAOs?\\ [0.5ex] 
% \hline
% \textbf{RQ3}: What are the implications of community\\ 
% behavior on the DAO network/Governance structure?\\[0.5ex] 
%  \hline
% \end{tabular}
% \caption{Our main research questions}
% \end{center}
% \end{table}





==> arxiv_2024_S&P_DAO-Paper_final/section/Related-Work.tex <==
\vspace{-2mm}
\section{Related Work}
\label{related_work}
\vspace{-2mm}
\subsection{History of DAOs}
\vspace{-2mm}
The concept of a DAO has existed since the mid-2010s~\cite{chohan2017decentralized}. \emph{The DAO} was originally designed as an investor-driven venture capital fund that relied on voting by investors to disburse funds to proposals submitted by contractors and vetted by curators~\cite{mehar2019understanding}. It operates as a transparent and democratically structured virtual platform, without physical addresses or formal managerial roles. Despite its potential of launching one of the largest crowdfunded campaigns ever seen~\cite{liu2021technology}, it was immediately hacked and drained of \$50 million in cryptocurrency~\cite{dhillon2017dao}, highlighting a mismatch between the system's openness and the potential for nefarious actions~\cite{liu2021technology, morrison2020dao, dupont2017experiments}. Yet, this should not conflate the broader category of smart contract based similar technologies, such as Dash governance~\cite{mosley2022towards}, Digix.io\footnote{Digix.io is a smart-asset gold-focused coin that seeks to match its value with the price of physical gold.}, Augur\footnote{Augur centers around the prediction markets and betting arenas where financial options and insurance markets can be developed.}, Uniswap\footnote{Uniswap is a crypto exchange based on smart contracts}. Many of these focused on blockchain-based assets and digital variants of existing socioeconomic instruments such as insurance, exchange markets, and social media~\cite{dupont2017experiments}. While some researchers argue that DAOs were initially limited to private capital allocation~\cite{chohan2017decentralized, trisetyarso2019crypto}, there is a growing trend to use DAOs in high-value data, and reputational-based systems~\cite{myeong2019administrative, barbosa2018cryptocurrencies,chohan2017decentralized}. The deterministic and non-probabilistic nature of smart contracts can be adapted~\cite{chatterjee2019probabilistic} towards these new paradigms based on the refinement of programming logic of organizational rules~\cite{ciatto2018blockchain}. 

Although it is difficult to describe DAOs as an organizational type~\cite{tse2020decentralised, trisetyarso2019crypto}, the conceptual basis of a DAO is its underlying ability within blockchain to provide a secure digital ledger that tracks financial interactions across the internet, bolstered against forgery by trusted timestamping and a distributed database. Users and practitioners who argue for decentralized and autonomous technologically-driven solutions have supported this idea to reflect and facilitate virtualization tendencies~\cite{ellul2019blockchain}. 
Unlike traditional capitalist organizations with undemocratic decision-making processes, where power is concentrated among boards, management, and shareholders, according to Marxist theory~\cite{bowles2012democracy}, DAOs offer a decentralized alternative, allowing for democratic decision-making through consensus protocols~\cite{dupont2017experiments}.
However, there has been the ever-continuing discussion around relegating management to pre-programmed rules, where transparency and efficiency are marked positives, but unstable security and low flexibility are the disadvantages~\cite{chohan2017decentralized}. 

%DAOs may be constructed without human managerial interactivity, provided that the underlying smart contracts are made robust and substantiated by Turing-complete mechanisms~\cite{dupont2017experiments}, extending the logic of the DAO along cryptoanarchist principles. 
%While the critique observed from Marxian theory towards capitalist organization is geared towards the non-democratic nature of decision-making within the boards, management, shareholder concentration, and the top-down directionality, DAOs provide a counterpoint to this skewed ownership and participation by facilitating decentralized execution of protocols through consensus. 

%Many of these offerings are centered around the evolution of blockchain-based assets and digital variants of existing socioeconomic instruments (insurance, exchange markets, and social media), but the ambitions of DAOs as organizations run on pre-programmed protocols are undoubtedly much greater~\cite{dupont2017experiments}. Gradually, projects were not only limited to smaller scale private capital allocation~\cite{risetyarso et al., 2019} as argued by some researchers~\cite{eiheiser et al., 2020; Myeong and Jung, 2019; Barbosa et al., 2018}. Some scholars see DAO-type usages in areas with sensitive data (such as genomics~\cite{ozercan2018realizing}), or just data with great value~\cite{Li et al., 2021} while others see usage in reputational-based systems~\cite{bellini2020blockchain}. Therefore, researchers suggested that the deterministic and non-probabilistic nature of smart contract \cite{Chatterjee et al., 2019a} can be adapted towards this new paradigms depending on the refinement of programming logic of organizational rules and regulations~\cite{iatto et al.,2018}. Yet, the idea was considered difficult to describe as an organizational type~\cite{Trisetyarso et al., 2019; Tse, 2020}, the conceptual basis of a DAO has been typologized by an underlying ability of blockchain technology to provide a secure digital ledger that tracks financial interactions across the internet and is bolstered against forgery by a method known as trusted timestamping and by dissemination of a distributed database. A further extension of the logic of the DAO, along cryptoanarchist principles, is that DAOs may be constructed in a manner that allows function without human managerial interactivity, so long as the underlying smart contracts are made robust and substantiated by Turing-complete mechanisms~\cite{dupont2017experiments}.

\vspace{-2mm}
\subsection{DAO in Context of Co-ordination
%DAOs \& Co-Ordination
}
%According to Ethereum's white paper by Buterin, a DAO is defined as a \emph{``virtual entity''} with members who can spend the entity's funds and modify its code~\cite{buterin2014next}. 
\vspace{-2mm}
DAOs enable individuals to coordinate and govern through self-executing rules on blockchain, without centralized control~\cite{buterin2014next}. While the primary objective of a DAO is to replicate traditional organizations with distributed decision-making by using blockchain technology, the precise definition of a DAO is currently contested~\cite{dupont2017experiments}. Some argue that all cryptocurrencies can be considered DAOs, while others propose that decentralized and autonomous governance structures could be considered the original DAOs~\cite{morrison2020dao}. As such, the specific tasks that require coordination within a DAO and what it means to \emph{``coordinate''} in this context of blockchain require further exploration.
%
There is a wealth of academic literature, even if those do not specifically mention the term \emph{``DAO''} by name, including economics theory of the firm~\cite{williamson2002theory}, public choice theory~\cite{shaw2002public}, and voting paradoxes~\cite{nurmi1999voting}. They analyze the behavior of voters, interest groups, politicians, and bureaucrats in shaping policy and outcomes, which is similar to the structure of DAOs. However, voting paradoxes and the Gibbard-Satterthwaite theorem~\cite{benoit2000gibbard} demonstrate that an individual's voting power can be affected by the voting system's structure and the distribution of voter preferences, and that there is no perfect voting system~\cite{satterthwaite1975strategy} that can consistently and accurately represent the preferences of voters. Furthermore, coordination in management science is critical to ensure that resources are used efficiently and that organizations work towards the same objectives~\cite{faraj2006coordination}. Performance metrics and feedback mechanisms~\cite{faraj2006coordination}, as well as computer-based coordination tools~\cite{fish1988quilt, stokols2008ecology}, are deemed to be necessary to track progress towards organizational goals.  
%Similarly, Computer-Supported Cooperative Work (CSCW) pointed out the need for emerging technologies to adopt computer-based tools and systems to facilitate and enhance communication, coordination, and collaboration\cite{fish1988quilt, stokols2008ecology}
Recent Literature on DAOs highlighted challenges in achieving similar goals and optimizing resources~\cite{baninemeh2023decision}, indicating for further investigation.
%Literature in Computer-Supported Cooperative Work (CSCW) has existing work for the design and development of computer-based tools and systems that can facilitate and enhance communication, coordination, and collaboration in work settings~\cite{fish1988quilt, stokols2008ecology}. 






\subsection{
%DAO As Autonomous Organization
Blurred Boundary of Autonomy in DAO: Human Involvement \& External Influence
}
\label{subsec:rw-autonomous}

%The emergence of DAOs has the potential to disrupt various industries beyond finance, including, a range of areas such as work, the arts, and governance, including the restructuring of the basis of democracy in human societies. Although these applications claim to be autonomous, human action is required to evolve them~\cite{wright2021measuring}. 

The concept of autonomy in DAOs has been a subject of ongoing discourse within technical, legal, and financial spheres~\cite{wright2021measuring, wright2021measuring}. The debate centers on whether DAOs should function as fully autonomous and automated entities, with no external parties involved in decision-making processes, or whether autonomy should be understood in a more nuanced way, emphasizing transparency and clear decision-making procedures~\cite{santana2022blockchain}.
%Some argue that DAOs should be fully autonomous and fully automated, with no external parties involved in decision-making processes~\cite{santana2022blockchain}. Others propose a more nuanced interpretation of autonomy, emphasizing transparency and clear decision-making processes.
Existing literature on autonomous agents, such as robots, mobile devices, as well as human-robot interactions, has identified various levels of autonomy, defined as the capacity to sense, plan, and act without human intervention or external control~\cite{sae2018taxonomy, elhannouny2019off, clough2002metrics, federal2015operation, huang2005autonomy,heckman1998liability,dowling2000intelligent}.
%and ethical and liability issues have been raised in relation to autonomous agent designs. 
In the case of Decentralized Organizations, it replaces a hierarchical structure managed by humans with a protocol specified in code and enforced on the blockchain, allowing for decentralized decision-making and controlling physical property. DAOs represent a unique combination of the concepts of Autonomous Agents (without human involvement) and Decentralized Organizations (without external influence), blurring the boundaries between the two.
Specifically, DAOs are entities that operate autonomously for certain tasks using smart contracts but also rely on hiring individuals to perform specific tasks that the automaton itself cannot perform, interacting according to their protocols~\cite{ethereum}.
%While, touches on both concepts of Autonomous Agent (without human involvement) involving AI and Decentralized Organizations (without external influence), it is not quite clear exactly where DAO sit
%Literature on other autonomous devices and applications (e.g. mobile devices, robots, and software agents) has proposed various levels of autonomy. For example, the levels of autonomy in automobiles have been sequenced as decreasing levels of human supervision~\cite{sae2018taxonomy}, and sea mobile device autonomy has been classified into four levels ranging from decision support to fully autonomous~\cite{elhannouny2019off}. 
%Air mobility taxonomy defines and sequences autonomy levels based on the complexity of the scenario and its computational task. 
%In the context of human-robot interactions, autonomy is defined as the extent to which a robot can sense, plan, and act in its environment without external control~\cite{clough2002metrics, federal2015operation, huang2005autonomy}.
%Autonomous software agent concepts have also been evolving, with various studies examining potential liability and ethical issues. 

%Various researchers have addressed potential liability and ethical issues arising from autonomous agent designs~\cite{heckman1998liability,dowling2000intelligent}. Pagallo provides a historical perspective on the liability issues arising from automation through to autonomous systems~\cite{pagallo2017automation}. Different studies propose different levels of autonomy to determine where a morally salient decision belongs on the ethical scale~\cite{dyrkolbotn2017classifying}.
Defining autonomy metrics for DAOs is challenging since existing taxonomies are often ambiguous and categorical rather than quantitative along a continuum~\cite{wright2021measuring}.  Decision-making scope and liability are the most generalizable dimensions, with domain-specific definitions being less easily generalizable. Prior research on autonomous agent designs has explored ethical and liability issues, including historical liability concerns from automation to autonomous systems~\cite{heckman1998liability,dowling2000intelligent,pagallo2017automation}, and proposed varying levels of autonomy for determining ethical significance~\cite{dyrkolbotn2017classifying}.
Themes that can be applied to DAOs include the degree of human supervision, decision-making roles, liability, and ethical considerations~\cite{haupt2019artificial}. 
%Brock distinguishes autonomy from decentralization in the context of individuals and organizations~\cite{brock2003autonomy}. 
Ladner et al. propose an index for local autonomy in European political entities~\cite{ladner2019local}. Other dimensions, such as those related to human development considerations, may be insightful with regard to artificial intelligence discussions~\cite{ryan2019brick}, but early DAOs are not assumed to require artificial intelligence. Of these dimensions, the notions of legal autonomy and financial autonomy would seem to be applicable in the context of DAOs. This is further complicated by regulatory proposals, such as the \emph{``Responsible Financial Innovation Act,''} which classifies DAOs as business entities for tax purposes~\cite{kramerresponsible}. Additionally, the governance models of DAOs are evolving, with emerging forms such as CityDAO which proposes to adopt a mayor-council model, where an appointed Mayor holds administrative and budgetary authority, an appointed Council holds legislative authority, and Professional Managers hold administrative authority~\cite{citydao}. 
%Furthermore, in Wyoming state, laws have been passed to establish a clear legal framework for the operation of DAOs and to make it easier for businesses to use blockchain technology~\cite{wyo}. These laws focus on providing a clear and predictable legal framework for the operation of DAOs, to make it easier for businesses to use blockchain technology, and to promote the autonomy of these organizations by providing a clear separation of assets, members, and management.
%\korn{I am also abit confused by this sentence->} 
%Moreover, the utilization of smart contracts raises questions regarding the nature of this activity as an organizational function and whether a higher degree of involvement is necessary. 
In this paper, we aim to understand the degree to which DAO operates with less human intervention and without undue external influence, potentially from corporate competitors or regulators.
%\anote{This is fairly shallow, can these questions connect to the specific RQs we do?} \tanusree{updated this paragraph to detail literature from different field on autonomy}


%In addition, integrating community decision-making on off-chain platforms with on-chain operations can present significant technical hurdles for DAOs. 
%\yujin{This is related to DAO autonomy? The difficulties in the integration between offchain and onchain operations hinder the autonomy of DAO? } \tanusree{yes, added the example of makerDAO}
%As previously reported in the literature~\cite{wang2019decentralized}, these obstacles include matters of contention, community discussions, and conflicts that may compromise the impartiality of decision-making processes.
%Recent research on MakerDAO suggests that a dominant voter coalition signals a degree of centralization in governance within the DAO, while also demonstrating the complicated influence that such voter coalitions can have on the Maker protocol~\cite{sun2022multiparty}. In addition, several tech reports and DAO experts have noted that competing interests or disagreements among members can stem from differences in opinions, values, goals, or incentives, resulting in non-optimal decisions for the DAO. However, it has been suggested that a diverse and inclusive membership can help mitigate the impact of biases on decision-making.
%\anote{What does this mean, conflicts can bias decision-making? Conflicts might be something interesting we can quantify?} \tanusree{updated, found one literature. we crawled online channel data for further analysis of conflict, not included in this paper. Conflicts may be a potential topic for discussion in this paper}
%\korn{Should law and regulations of DAO be a separate paragraph?}


%However, the societal impact of these technologies is significant, including considerations around safety, security, privacy, and consequences of failure. It is important to measure autonomy in order to raise consumer awareness as these autonomous devices and applications scale out to mass markets.  As these applications of DAOs scale out to mass-market consumers it becomes important for consumers to have realistic expectations regarding the autonomy of DAOs for everyday commercial transactions. The development and disclosure of DAO autonomy metrics would be helpful as a means to quantify the degree of autonomy for assessment of DAO designs and tracking of operating DAO performance.



%There exists technical challenges around if DAO need to be fully autonomous and fully automated (i.e. the DAO should operate without any external parties), or whether the concept of ``autonomy'' should be interpreted more clearly/ transparency \cite{}. There are discussion around lack of connection among community decision in off-chain platform snapshot and on-chain operations. Also, empirical studies with Twitter data and discord conversations hinted the influence of community discussion, contested facts and conflicts to the outcome of decision making and how those can bias some decision making in the DAO proposal and voting etc. Some researches also explored legal challenges involving the act of transacting with a smart contract qualify as an organisational activity, or whether a stronger degree of involvement is necessary in legal aspects, such as having a governance model or collective interactions amongst participants \cite{}. Autonomy of DAOs further complicate the the new ``Responsible Financial Innovation Act'' proposal has some rules for DAOs, e.g., in some cases, DAOs are considered business entities for tax purposes \cite{}.. Besides traditional proposers, voters, there are emerging forms of governance models, e.g., CityDAO is proposing to adopt the mayor-council model: ``Mayor-Council governance with an appointed Mayor holding administrative and budgetary authority, an appointed Council with legislative authority, and Professional Managers who hold administrative authority.''  Another example towards the regulatory building- Wyoming state has passed several laws that aim to establish a clear legal framework for the operation of DAOs and to make it easier for businesses to use blockchain technology. These laws focus on providing a clear and predictable legal framework for the operation of DAOs, to make it easier for businesses to use blockchain technology, and to promote the autonomy of these organizations by providing a clear separation of assets, members, and management. This includes the formation of a new type of limited liability company (LLC) called a Series LLC, defining "utility tokens" as a digital asset that is not a security and that is used to purchase a good or service, or to access a platform or application, and providing regulatory oversight for banks and trust companies that custody digital assets including DAOs' assets, among others.
%Wyomin state has passed several laws that aim to provide a clear legal framework for the operation of DAOs, and to make it easier for businesses to use blockchain technology Laws aim to provide a clear and predictable legal framework for the operation of DAOs, to make it easier for businesses to use blockchain technology, and to promote the autonomy of these organizations by providing a clear separation of assets, members, and management

%\andrew{We could talk about the new DAO laws in Wyoming and what they aim to achieve.}
    
  % \yang{the new ``Responsible Financial Innovation Act'' proposal has some rules for DAOs, e.g., in some cases, DAOs are considered business entities for tax purposes}

%\yang{besides traditional proposers, voters, there are emerging forms of governance models, e.g., CityDAO is proposing to adopt the mayor-council model: ``Mayor-Council governance with an appointed Mayor holding administrative and budgetary authority, an appointed Council with legislative authority, and Professional Managers who hold administrative authority.''}


\iffalse
\subsection{DAO Incentives \& Participation}

In blockchain ecosystems, designing a proper incentive system has always been regarded as an important but challenging problem. For example, the optimal incentives in consensus protocols of blockchain systems still remain an open problem even though many researchers and developers have actively attempted to analyze and improve the current incentive systems \cite{kwon2019impossibility, gencer2018decentralization, li2020comparison, huang2021rich,lin2021measuring, brunjes2020reward, saad2021pos}. DAO governance is similar to the consensus protocols, given that they both should encourage many entities to participate evenly. Therefore, similar discussions also appear in the DAO community. 

Healthy and robust DAO systems are generally considered ones in which many entities evenly participate. One of the most critical points that enable healthy and robust DAOs is to have a proper incentive\footnote{https://blog.aragon.org/incentive-design-tooling-for-daos/}. 
Our paper will confirm that many existing DAOs struggle with poor decentralization or a low participation rate, which implies that current DAOs lack proper incentive systems~\cite{kaal2021decentralized}. 
Currently, it is unclear what the optimal incentive designs are, and even there has been yet little research on DAO incentives \cite{liu2022user}. Some studies \cite{liu2022user,guidi2020graph} show that not only monetary rewards but also social rewards like reputation and approval can promote the engagement of users, by analyzing the Steemit system, an example of DAOs. On the other hand, several studies also point out the poor decentralization or unfairness of Steemit~\cite{li2019incentivized, guidi2020graph, guidi2021analysis}. Another paper~\cite{gao2022true} focused on the NFT marketplaces to see if the token incentives can draw active participation of users in the DAO environment. Although they confirm the helpfulness of token incentives to induce user participation, our analysis results also cast doubt on that the token incentives alone can lead to healthy and robust DAO systems. In summary, there remain many challenges to what the proper incentives of DAOs are. 
\fi

==> arxiv_2024_S&P_DAO-Paper_final/section/Results.tex <==
\vspace{-2mm}
\section{RQ2: Decentralization of DAOs}
\label{section5}
\vspace{-2mm}

In this section, we investigated the level of decentralization in the current DAOs with respect to voting and proposal.

\vspace{-2mm}
\subsection{Voting Patterns Among DAO Holders}
\vspace{-2mm}

%To understand the involvement of various stakeholders in the DAO governance system, 
%We conducted analyses to examine the interactions among DAO holders to identify similarities and differences based on voting patterns for proposals. 
Our interview study (section~\ref{interview}) highlights the limitation that token-based governance disincentivizes grassroot holders from participating in the decision-making process, particularly with regard to the tendency for core or managerial teams to hold a majority of tokens, leading to centralized decision-making by a small group. 
Given this, we examine the interaction between different DAO holders and present clustering of holders based on their voting decisions for different proposals. 
%\yang{need to articulate why this is related to decentralization. or if a DAO is decentralized, what you'd expect to see the voting patterns. guide readers thru our analysis}\tanusree{updated}. 
We also analyze the voting patterns of large token holders (whales) to establish their positionalities and investigate whether their voting patterns align with broader community. Given that greater token holdings represent greater influence of holders in DAO voting systems, if voting patterns of whale addresses do not align with grassroots users or their voting patterns only have similarities among themselves, it implies that the grassroots users are marginalized, suggesting poor decentralization.
%We hypothesize that if whale addresses hold a majority of tokens and their voting patterns do not align with grassroots users or their voting patterns only have similarities among themselves, the DAO is likely to have poor decentralization. 
%\yang{let's connect to decentralization. so is this the relationship between decentralization and DAO proposal outcome?} \tanusree{relationship between decentralization with voting pattern- when whales holding majority of token to indicate poor decentralization. updated}

\begin{figure*}[!htb]
\begin{subfigure}{0.20\textwidth}
  \includegraphics[width=\linewidth]{images/f_bitDAO.png}
  \caption{BitDAO}\label{fig:bit_image1}
\end{subfigure}\hfill
\begin{subfigure}{0.20\textwidth}
  \includegraphics[width=\linewidth]{images/compound.png}
  \caption{CompoundDAO}\label{fig:comp_image2}
\end{subfigure}\hfill
\begin{subfigure}{0.20\textwidth}%
  \includegraphics[width=\linewidth]{images/f_assange_net.png}
  \caption{AssangeDAO}\label{fig:assange_image3}
  \end{subfigure}\hfill
\begin{subfigure}{0.20\textwidth}%
  \includegraphics[width=\linewidth]{images/f_bankless_net.png}
  \caption{BanklessDAO}\label{fig:assange_image3}
  \end{subfigure}\hfill
\begin{subfigure}{0.20\textwidth}%
  \includegraphics[width=\linewidth]{images/f_krause_net.png}
  \caption{KrauseHouse}\label{fig:assange_image3}
\end{subfigure}
\caption{DAO holders' voting behavior for different proposals are displayed as community graphs. A cluster is defined based on their voting behavior where 1: voted for certain proposal, -1: voted against certain proposal. The colored polygons in subgraphs (a), (b), and (c) represent the nodes with similar voting behavior. There are some overlapped colored regions which indicate that nodes in those clusters have some voting similarity with nodes in other cluster.
For example, figure (a) shows no overlapped clusters because the nodes from different clusters do not share any similar voting behavior. In contrast, figure (b) shows the cluster containing yellow nodes has a overlapped region with the cluster containing red nodes due to some voting similarity (at least one voting similarity between nodes/addresses). 
\vspace{-2mm}} 
\label{cluster1}
\end{figure*}

\begin{figure*}[!htb]
\begin{subfigure}{0.25\textwidth}
  \includegraphics[width=\linewidth]{images/Compound-w.png}
  \caption{CompoundDAO Voting Pattern with directed graph. Each edge means the two nodes voted the same way to a proposal.}\label{fig:c-1}
\end{subfigure}\hfill
\begin{subfigure}{0.25\textwidth}
  \includegraphics[width=\linewidth]{images/compound-org.png}
  \caption{CompoundDAO Voting Pattern of different type of users. Blue represents Industry. Yellow: non profit. Red: Educational Institute. Green: individual users, big green nodes are KOLs. %This graph is generated by running clustering first, and identify main nodes in each cluster and check which type these main nodes belong to.
  }
  \label{fig:c-2}
\end{subfigure}\hfill
\begin{subfigure}{0.25\textwidth}%
  \includegraphics[width=\linewidth]{images/comp-w.png}
  \caption{CompoundDAO Whale address. Industry:blue, Non Profit:green, Educational Institute:red, Key Opinion Leader:yellow }\label{fig:c-3}
\end{subfigure}
\caption{%In (1d) edges are coloured according to the project the transferred token belongs to
We present CompoundDAO as an example to demonstrate the result of the first hypothesis, H1. Here the size of the nodes is directly proportional to their input degree (i.e., the larger a node, the more tokens it has accumulated in the DAO). Blue nodes represent industry,  green for non-profit organizations, red for educational institutes, and yellow for key opinion leaders (KOLs). 
We found 32 addresses with a large threshold of Compound token holding. 
%Based on coinmaketcap and intotheblock, the addresses above this threshold are defined as whale addresses for CompoundDAO. 
Figure 2c shows that whale addresses from industry, KOLs and educational institutes tend to have similar voting behavior.\vspace{-2mm}}  %\yang{what's the main take-away from these graphs?} \tanusree{updated}}
\label{cluster-2}
\end{figure*}


\begin{table*}[]
\scriptsize

\begin{tabular}{lllllllllll}
\hline
DAOs        & \begin{tabular}[c]{@{}l@{}}Freq of \\ community\end{tabular} & Vertics & Edge    & Diameter & \begin{tabular}[c]{@{}l@{}}Mean\\ Distance\end{tabular} & %\begin{tabular}[c]{@{}l@{}}Degree \\ %Reciprocity\end{tabular} &
\begin{tabular}[c]{@{}l@{}}Degree \\ Transitivity\end{tabular} & \begin{tabular}[c]{@{}l@{}}Degree \\ Assortativity\end{tabular} & \begin{tabular}[c]{@{}l@{}}Degree \\ Centralization\end{tabular} & \begin{tabular}[c]{@{}l@{}}Betweenness \\ Centralization\end{tabular} & \begin{tabular}[c]{@{}l@{}}Closeness \\ Centralization\end{tabular} \\
\hline
Bit         & 4                                                            & 283     & 26985   & 4        & 1.33                                                                                                                & 0.93                                                           & 0.616                                                            & 0.31                                                             & 0.04                                                                  & 0.44                                                                \\
Assange     & 6                                                            & 1065    & 380410  & 3        & 1.33                                                                                                                & 0.87                                                           & 0.04                                                           & 0.32                                                             & 0.002                                                                 & 0.45                                                                \\
PoH         & 5                                                            & 3084    & 1403628 & 4        & 1.7                                                                                                              & 0.66                                                           & -0.2                                                           & 0.68                                                             & 0.008                                                                 & 0.77                                                                \\
Bankless    & 5                                                            & 3139    & 1758001 & 3        & 1.64                                                                                                              & 0.59                                                           & 0.09                                                           & 0.64                                                             & 0.004                                                                 & 0.24                                                                \\
KrauseHouse & 4                                                            & 587     & 63713   & 3        & 1.63                                                                                                              & 0.74                                                           & 0.07                                                           & 0.54                                                             & 0.019                                                                 & 0.59                                                                \\
Compound    & 10                                                           & 2482    & 378635  & 4        & 1.65                                                                                                              & 0.75                                                          & 0.026                                                          & 0.75                                                             & 0.09                                                                  & 0.72                                                                \\
LivePeer    & 2                                                            & 367     & 21802   & 2        & 1.68                                                                                                             & 0.68                                                           & -0.2                                                           & 0.67                                                             & 0.04                                                                  & 0.79                                                                \\
MGD         & 2                                                            & 15      & 56      & 5        & 1.49                                                                                                                & 0.66                                                           & -0.2                                                            & 0.32                                                             & 0.09                                                                  & 0.42                                                                \\
Moloch      & 2                                                            & 14      & 50      & 3        & 1.45                                                                                                              & 0.65                                                           & -0.29                                                           & 0.37                                                             & 0.13                                                                  & 0.5                                                                 \\
dxDAO       & 4                                                            & 270     & 35520   & 2        & 1.02                                                                                                           & 0.99                                                           & 0.60                                                           & 0.32                                                             & 0.01                                                                  & 0.03          \\                                                     
\hline
\end{tabular}
\caption{Network Graph connectivity and clustering statistics for each DAOs in terms of reciprocity, transitivity and assortativity, vertices, edges, diameter, mean distance}
\label{tab:graph}
\end{table*}

\begin{comment}
    

\begin{table*}[]
\scriptsize
\begin{tabular}{@{}llllllll@{}}

%\rowcolor[HTML]{A2C4C9} 
\hline
\textbf{DAOs}     & \textbf{\begin{tabular}[c]{@{}l@{}}Freq of \\ community\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}Degree \\ Reciprocity\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}Degree \\ Transitivity\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}Degree \\ Assortativity\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}Degree \\ Centralization\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}Betweenness \\ Centralization\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}Closeness \\ Centralization\end{tabular}} \\ \midrule
\hline
BitDAO            & 4                                                                     & 1                                                                      & 0.93                                                                    & 0.31                                                                     & 0.31                                                                      & 0.04                                                                           & 0.44                                                                         \\
AssangeDAO        & 6                                                                     & 1                                                                      & 0.87                                                                    & -0.04                                                                    & 0.32                                                                      & 0.002                                                                          & 0.45                                                                         \\
Proof of Humanity & 5                                                                     & 1                                                                      & 0.66                                                                    & -0.15                                                                    & 0.68                                                                      & 0.008                                                                          & 0.77                                                                         \\
BanklessDAO       & 5                                                                     & 1                                                                      & 0.59                                                                    & -0.09                                                                    & 0.64                                                                      & 0.004                                                                          & 0.24                                                                         \\
KrauseHouse       & 4                                                                     & 1                                                                      & 0.74                                                                    & -0.07                                                                    & 0.54                                                                      & 0.019                                                                          & 0.59                                                                         \\
CompoundDAO       & 10                                                                    & 1                                                                      & 0.59                                                                    & -0.004                                                                   & 0.75                                                                      & 0.09                                                                           & 0.72                                                                         \\
LivePeer          & 2                                                                     & 1                                                                      & 0.68                                                                    & -0.15                                                                    & 0.67                                                                      & 0.04                                                                           & 0.79                                                                         \\
Meta Gamma Delta  & 2                                                                     & 1                                                                      & 0.66                                                                    & -0.2                                                                     & 0.32                                                                      & 0.09                                                                           & 0.42                                                                         \\
MolochDAO         & 2                                                                     & 1                                                                      & 0.65                                                                    & -0.29                                                                    & 0.37                                                                      & 0.13                                                                           & 0.5                                                                          \\
dxDAO             & 4                                                                     & 1                                                                      & 0.99                                                                    & 0.48                                                                     & 0.02                                                                      & 0.01                                                                           & 0.03                                   \\ 
\hline
\end{tabular}
\caption{Network Graph connectivity and clustering statistics for each DAOs in terms of reciprocity, transitivity and assortativity}
\end{table*}
\end{comment}



\begin{comment}

\begin{figure*}[!htb]
\minipage{0.25\textwidth}
  \includegraphics[width=\linewidth]{BitDAO.png}
  \caption{BitDAO Voting Pattern}\label{fig:awesome_image1}
\endminipage\hfill
\minipage{0.25\textwidth}
  \includegraphics[width=\linewidth]{compound.png}
  \caption{CompoundDAO Voting Pattern}\label{fig:awesome_image2}
\endminipage\hfill
\minipage{0.25\textwidth}%
  \includegraphics[width=\linewidth]{assange.png}
  \caption{AssangeDAO Voting Patterns}\label{fig:awesome_image3}
\endminipage
\caption{DAO holders' voting behavior for different proposals are displayed as community graphs. The cluster is defined based on their voting behavior where 1: voted for certain proposal, -1: voted against certain proposal and 0: no vote for certain proposal. In (1d) edges are coloured according to the project the transferred token belongs to} \yang{i don't understand what the edge represents}
\label{cluster1}
\end{figure*}

\begin{figure*}[!htb]
\minipage{0.25\textwidth}
  \includegraphics[width=\linewidth]{Compound-w.png}
  \caption{CompoundDAO Voting Pattern with directed graph}\label{fig:c-1}
\endminipage\hfill
\minipage{0.25\textwidth}
  \includegraphics[width=\linewidth]{compound-org.png}
  \caption{CompoundDAO Voting Pattern of different type of users. Blue represent Industry, yellow: educational institute, red: non profit organization , green  individual users}
  \label{fig:c-2}
\endminipage\hfill
\minipage{0.25\textwidth}%
  \includegraphics[width=\linewidth]{compound-whale.png}
  \caption{CompoundDAO Whale address \yang{where is this graph?}}\label{fig:c-3}
\endminipage
\caption{Example: We present CompoundDAO as an example to demonstrate the result of the first hypothesis, H1. In the Figure, the size of the nodes is directly proportional to their input degree (i.e., the larger a node, the moretokens it has accumulated in the DAO). We found 32 addresses with large threshold of Compound token holding (10K-100K+). Based on coinmaketcap \footnote{https://coinmarketcap.com/} and intotheblock{https://www.intotheblock.com/}, the addresses in this threshold are defined as whale addresses for CompoundDA.}
\label{cluster2}
\end{figure*}

\end{comment}

\vspace{-2mm}
\subsubsection{Graph Model}
We developed network graphs to understand DAO holders' voting patterns across different proposals, considering their voting weights. %and patterns of voting for different proposals. 
In the graphs, each node $v_i (\in V)$ represents a unique Ethereum address, where $V$ indicates the full set of nodes. Nodes are connected via an edge if they voted the same way (e.g., voted yes) in the same proposal, and $E$ denotes a set of edges $\{(v_{i}, v_{j}) | v_{i}, v_{j}\in V\}$, where $(v_{i}, v_{j})$ indicates an edge between $v_i$ and $v_j.$
The graph structures of DAOs (Figures~\ref{cluster1} and \ref{cluster-2}) are derived using the walktrap algorithm, commonly used to identify communities in networks via random walks~\cite{petrochilos2013using}. %Here, the random walks are then used to compute distances between nodes. The voting behaviors of DAO holders are calculated in a weighted graph $G(V,E)$ with a full set of nodes $V$ and edges $E$ = ${(v_{i}, v_{j})}$ for $v_{i}, v_{j}\in V$.
Here, the random walks are also used to compute distances between nodes. Therefore, we calculated the optimal similarities and differences of voting behaviors of DAO holders in a weighted graph $G(V,E)$.
%\yujin{calculate the voting behaviors? or calculate the similarities between the voting behaviors?} 
%, where $V$ and $E$ indicate the full set of nodes and a set of directed edges $\{(v_{i}, v_{j}) | v_{i}, v_{j}\in V\}$, respectively. Note that $(v_{i}, v_{j})$ represents a directed edge from $v_i$ to $v_j.$
%\yujin{Please check whether the revised version is correct.}

The colors represent clusters related to \textit{``VoterType''} who vote in similar ways for different proposals\footnote{We use the igraph R package to calculate the different clusters: https://igraph.org/r/}. 
%Each node $v_i (\in V)$ represents a unique Ethereum address. %and each directed edge $e_{i,j}^k \epsilon E$ represents a single address to a proposal voting decision. 
%and nodes are connected to other node (ethereum address) via an edge if they voted the same way in the proposals.
%
%from other accounts with similar voting patterns for different proposals. 
%\update{
If two nodes have more than one same vote, they are more likely to be in the same cluster. 
%However, nodes having only one same vote intersection will likely be in different clusters. 
%
To construct a voting network graph, we first created a matrix\footnote{We used an incidence matrix to make a bipartie graph since the number of rows is different than the number of columns. Within the $incidence matrix$, there will be an adjacency matrix with similar number of columns and rows.} whose entity indicates a vote on a certain proposal done by an address.
%For each vote, an edge parameter indicates a voting direction; 
Entity values 1 and -1 imply a vote for and against a certain proposal, respectively. 
Based on the matrix, we built an adjacency matrix where columns and rows represent ``Votes'' and ``Addresses'', respectively. Then we constructed the bipartite graph between ``Address'' and ``Votes'' from the adjacency matrix. In the graph, an edge between Addresses and Votes indicates that an address has voted either against or for the proposals. 
%We used an incidence matrix to make a bipartie graph since the number of rows are different than the number of columns. Within the $incidence matrix$, there will be an adjacency matrix with similar number of columns and rows. \yujin{Can we remove this?}

Further, we present the community cluster with voting weight $w(v_{i}, v_{j})$, 
%
%Another parameter that we should consider is the voting weight, %$w(v_{i}, v_{j}^k)$,\yujin{$v_{j}$ instead of $v_{j}^k$?} 
which corresponds to the token amount each address delegated for themselves or others to perform the transaction (i.e., to vote for the proposal). 
%Note that the token amount is interpreted as voting power in a general DAO system.
%where each node is weighted by the voting amount they delegated for different proposals. 
We calculated the weight of each address by averaging the voting weight (or token amount) delegated to the address for each proposal. Nodes are sized by the number of votes/tokens they delegated; that is, larger nodes represent more highly delegated token accounts (Figure~\ref{cluster-2}). 
%In the following sections, we will analyze the nodes with more tokens in their network, and describe the positionality of those users within the DAO community space. %Mainly- 
%Thus, the hypothesis from our initial exploration of DAO holders' voting behavior and the further analysis to support this hypothesis can be found in ~\ref{h1}- 

% \begin{center}
% \begin{tabular}{|c |} 
%  \hline
% %\textbf{H1}: Whale voter addresses in DAOs tend to\\
% %agree with the broader community or they are people's \\
% %representative in terms of their voting behavior. \\ [0.5ex] 
% Which DAO holders tend to vote the same way on \\proposals? Does this voting patterns impact the DAO\\ proposal success
% and overall governance? \\
%  \hline

% \end{tabular}
% \end{center}


%\subsubsection{Graph Statistics: Patterns of Voting Networks of DAO holders}
\vspace{-2mm}
\subsubsection{Patterns of Voting Networks} %of DAO holders}

%{\bf Basic Quantities.} 
We present the main static properties of the constructed graphs. Table~\ref{tab:graph} summarizes the network properties of 10 DAOs: number of nodes and edges, diameter, mean distance, degree distributions, density, component clustering coefficients, and assortativity. 
Note that here we considered only addresses with an edge by eliminating null votes made by different addresses (i.e., discarding addresses that have not voted on any proposal). %This allows us to discover and analyze the behavior of communities participating in voting for different proposals.
%
%Only connections between two addresses in terms of ``voted for: 1'' and ``voted against: -1'' have been considered in this statistics. We did so because the main objective of this work is to discover and analyze the behavior of communities participating in voting for different proposals. Thus, we attempted to eliminate the biases by discarding the null voting made by different addresses (null or 0 voting refers to addresses who have not voted for certain proposals where participants could have different reasons for not voting for proposals). Within that, we calculated the distribution of node in-degrees and the flows of tokens within the network without disrupting connectivity and clustering analysis.
%Different parameters, discussed in the Table ~\ref{Tab:Tab1} and \ref{Tab:Tab2}, allow us to calculate the distribution of node in-degrees and the flows of tokens within the network without disrupting connectivity and clustering analysis.

%Visual idea of the structure of these graphs are presented in Figure~\ref{cluster1} and Figure~\ref{cluster2}. 
%The network graphs of BitDAO, CompoundDAO, AssangeDAO, BanklessDAO, and KrauseHouse are shown in Figure~\ref{cluster1}. The size of each node size is proportional to its input degree (i.e., the larger a node, the more tokens it has accumulated the DAOs). 
In Figure~\ref{cluster1}, the clusters are colored based on the optimal similarity of voting behaviors and the distance between the nodes. The overlapped regions of colored polygons indicate that there is at least one voting similarity between the nodes in one cluster and the others. In BitDAO, nodes in specified clusters have very few similarity in voting with other clusters, which results in comparatively less overlapping regions in Figure~\ref{fig:bit_image1}. On the other hand, the CompoundDAO network (Figure~\ref{fig:comp_image2}) has a total of 10 clusters, where some nodes in clusters have at least one similar voting with nodes in other clusters. For AssangeDAO (Figure~\ref{fig:assange_image3}), there are a total of six clusters, and most nodes have at least one voting similarity with other clusters. 
As such, one can see the significant difference in the network structures between DAO, which implies heterogeneous community voting behaviors. 
In contrast, we observed less cluster diversity in proof of humanity where the number of voters are second highest, however, voters tend to have similar voting patterns %maintaining the consistency across different proposals
(Figure~\ref{cluster-new} in Appendix). Meta Gamma Delta, Moloch, Livepeer, dxDAO tend to follow the similar trend.


\noindent\textbf{Connectivity and clustering properties.}
The assortativity coefficient~\cite{meghanathan2016assortativity} measures the homophyly level of the graph (i.e., how nodes are connected for a given property), and it ranges in $[-1,1]$. More specifically, according to \cite{meghanathan2016assortativity}, a graph is said to be strongly assortative, weakly assortative, neutral, weakly disassortative, and strongly disassortative, if the assortativity coefficient falls into the ranges $[0.6,1]$, $[0.2,0.6)$,$(-0.2,0.2)$,$(-0.6,-0.2]$, and $[-1,-0.6]$, respectively. 
%Table~\ref{tab:graph} illustrates the assortativity for DAO voting behavior graphs. 
%\dawn{it's helpful to explain these concepts in more detail.} \tanusree{updatedwith more details for interpretation}
Table~\ref{tab:graph} shows that majority of the DAO, including CompoundDAO, Krausehouse, Bankless and Assange, PoH to be neutrally assortative while BitDAO and dxDAO that are strongly assortative indicating that the nodes tend to be connected to other nodes with similar properties. However, in case of neutral assortativity, 
%the nodes are either well-mixed and highly connected facilitating information diffusion among nodes with different properties or can also indicate lack of structure or organization in the network. In other words, 
many DAO do not have the trend that members vote the same way as others with similar characteristics to them. We further illustrate this property in conjuction with degree centrality where we observed PoH, Bankless, Compound, Livepeer having degree centralization value above 0.6 indicating a significant concentration of node degrees. None of the DAO has degree centralization value below 0.3. 
The transitivity coefficient (also known as a clustering coefficient) measures the probability for nodes connected via multiple edges to be adjacent; in other words, if there are two links $(v_{i},v_{j})$ and $(v_{j},v_{k})$, what the probability of there being a link $(v_{i},v_{k})$ is. Table~\ref{tab:graph} illustrates various levels of transitivity across DAOs and the value is quite high. dxDAO has the highest transitivity at 0.99, implying that similarity in voting behaviors between nodes connected to other addresses is 99\%, BitDAO which in 93\%, AssangeDAO(87\%), CompoundDAO(75\%), KrauseHouse(74\%). PoH, Livepeer, MGD and Moloch have the probability for nodes connected via multiple edges 65-68\%. 
 %for CompoundDAO, it is 0.59, indicating that similarity between nodes (addresses) is 59\%. 
%The reciprocity coefficient measures the proportion of mutual connections on a directed graph. In other words, it estimates the probability that for given an edge $e(v_{i},v_{j})$, its reciprocal $e(v_{j},v_{i})$ also exist. From Table~\ref{tab:graph}, we can see that the reciprocity level for CompoundDAO is $1$, indicating that all addresses have similarity and both directional edges. \korn{I'm a bit lost here. I thought the directed graph is constructed such that an edge $(v_i, v_j)$ exists if the two addresses voted the same way for a proposal. Then, it would always be the case that if edge $(v_i, v_j)$ exists, then edge $(v_j, v_i)$ also exists?}
%\yujin{Because the considered graph is undirected, we should remove reciprocity.} 


We further provide a detailed examination of the voting network characteristics of various DAOs. Specifically, our analysis of the CompoundDAO protocol revealed high similarities in voting behaviors among grassroot users. Additionally, we identified one cluster composed of nodes with higher token weight (referred to as \emph{whale addresses}) that exhibit similar voting patterns. These nodes will be discussed in further detail in Section~\ref{h1}. Our analysis of the BitDAO also revealed similar voting patterns among nodes with higher token holdings, with less cluster distance and a tendency to vote in a similar manner. However, some higher token holders in these DAOs tend to be representative of grassroots compared to those in the CompoundDAO, although they remain polarized \footnote{Polarized voting refers to the tendency for dao voters to align themselves with clusters while token holdings dictate this polarization %one political party. In this context, token holdings dictate this polarization
}. We also observed significant overlaps in voting behaviors among different token holders in dxDAO, with only a few proposals resulting in significant voting leading to two small clusters. Similar patterns were observed in the AssangeDAO and BanklessDAO, with polarized voting behaviors among token holders. 
%In the case of the AssangeDAO, we observed a significant split in the community, with token holdings and voting patterns dictating their positions within the DAO.


%\yujin{Need to explain more what people representative means.} 

%\yujin{Need to explain what ``polarized'' means. It means the voting patters are significantly divided?} 

In contrast, our analysis revealed a more equitable distribution of voting patterns among different types of token holders for the Proof of Humanity DAO.
%\yujin{To avoid some confusion, how about saying less biased distribution(?) instead of better decentralization? } 
It might be because majority of the token holders ($>99\%$) in this DAO are grassroot users.
%\korn{Is this because one address gets 1 vote in PoH?}\tanusree{no, becuase 99\% has 1 token, rest have token from 2-35} 
For Livepeer, we found two main different types of voting behaviors with small overlaps regardless of the token holdings of voters, implying better decentralization and less biased voting patterns dictating upon token holding status. Finally, Meta Gamma Delta (MGD) and MolochDAO, we can not say that their decentralization level is high due to the small number of voters, however, token holding didn't dictate the voting patterns. 

%showed higher similarity of voting behaviors across various nodes, leading to better decentralization and less polarized
%voting decision. Here, note that we do not say that their decentralization level is high due to the small number of voters.
%\yujin{So what is the implication of Livepeer?}

%\dawn{in general, it's helpful to explain more clearly what we are measuring and what are ideal characteristics of decentralized DAOs.} \tanusree{added in 6.1}

\begin{tcolorbox}[width=\linewidth, colback=white!95!black, boxrule=0.5pt, left=2pt,right=2pt,top=1pt,bottom=1pt]
\stepcounter{observation}
{\bf Takeaways \arabic{observation}:}
{CompoundDAO, AssangeDAO, Bankless, and Krausehouse protocols exhibit high polarization based on token holdings while
%BitDAO and dxDAO show slightly better distribution. 
Proof of Humanity, MGD, and Moloch protocols exhibit more equitable distribution.
%of voting patterns regardless token. 
%Governance tokens of CompoundDAO, AssangeDAO, Bankless, BitDAO, Livepeer, and Krausehouse are traded on secondary markets, while dxDAO's voting power is distributed by participation. Proof of Humanity has $\geq$ 99\% of voters with one vote, MGD and Moloch are based on shares, making it impossible to trade voting power in the market.

}

\end{tcolorbox}


%\yang{I'm still not completely clear what each of these network metrics mean in the context of DAO: e.g., assortativeness, coreness, reciprocity. For a successful or healthy DAO, should these values be high or low?}


\subsubsection{Positionality of Whale Addresses}
\label{h1}


%To this end, we first calculate Pagerank and coreness values~\cite{liu2existence015core} of nodes in DAO systems. Pagerank is generally used in web network graphs to estimate the importance of each node. On the other hand, coreness is used to identify closely interconnected groups within a network; a k-core indicates a (maximal) group of entities, all connected to at least k other entities in the same group. Figure~\ref{ccdf} shows the Complementary Cumulative Distribution Function (CCDF: basically the likelihood that the random variable is above a particular level, defined as $1-CDF$) of both Pagerank and coreness values for the CompoundDAO network graph. 
%The results show the presence of nodes that are more important than others. Specifically, the Pagerank distribution shows a significant bias of node influences. These networks also have cores of degrees equal to 100, with a very high probability, which implies the existence of high coreness nodes \cite{liu2015core}. 
%We investigate the existence of whale addresses in DAO systems. To this end, we first calculate Pagerank and coreness values~\cite{liu2015core} of nodes in DAO systems. Pagerank is generally used in web network graphs to estimate the importance of each node. On the other hand, coreness is used to identify closely interconnected groups within a network; a k-core indicates a (maximal) group of entities, all connected to at least k other entities in the same group. Figure~\ref{ccdf} shows the Complementary Cumulative Distribution Function (CCDF: basically the likelihood that the random variable is above a particular level, defined as $1-CDF$) of both Pagerank and coreness values for the CompoundDAO network graph. The results show the presence of nodes that are more important than others. Specifically, the Pagerank distribution shows a significant bias of node influences. These networks also have cores of degrees equal to 100, with a very high probability, which implies the existence of high coreness nodes \cite{liu2015core}. 
%It must be noted that, as demonstrated in \cite{liu2015core}, nodes with high coreness are not always influencers, although it is highly likely that influencer nodes are high coreness nodes.
%yujin{Can we remove this?}

\iffalse
\begin{figure}[!htb]
\minipage{0.23\textwidth}
 \includegraphics[width=\linewidth]{images/comp-pagerank.png}
  \subcaption{CompoundDAO Pagerank}\label{fig:pagerank}
\endminipage\hfill
\minipage{0.23\textwidth}%
  \includegraphics[width=\linewidth]{images/comp-coreness.png}
  \subcaption{CompoundDAO Coreness}\label{fig:c-1}
\endminipage
\caption{Graph connectivity values in terms of Complementary Cumulative Distribution Function (CCDF) Pagerank and coreness distributions.
%\yujin{It would be better to increase the x and y axes font sizes. }
}
\label{ccdf}
\end{figure}
\fi

%The power-law results described in Section V-B have been obtained using the poweRlawpackage in 

% \begin{figure}%
%     \centering
%     \subfloat[\centering Coreness]{{\includegraphics[width=5cm]{images/comp-coreness.png} }}%
%     \qquad
%     \subfloat[\centering PageRank]{{\includegraphics[width=5cm]{images/comp-pagerank.png} }}%
%     \caption{Graph connectivity values in term of Complementary Cumulative Distribution Function (CCDF) pagerank and coreness distributions. \tanusree{this is only for CompoundDAO now. I will add other 5 DAOs in the same plot with different color} }%
%     \label{fig:cp}%
% \end{figure}

%We investigate the existence of whale addresses in DAOs. 
We identify the whale addresses in different DAO by using Complementary Cumulative Distribution Function (CCDF: the likelihood that the random variable is above a particular level, defined as $1-CDF$), based on DAO holders' token holdings. %referred from coinmarketcap~\cite{coinmarketcap}. 
As an example, we present CompoundDAO's member addresses for the network analysis. Table~\ref{tab:graph-whale} in Appendix present number of whale for 10 DAOs and other network properties. We find that there are $2482$ unique addresses in CompoundDAO, from which $32$ addresses (Figure~\ref{fig:c-3} are identified as whale addresses ($100k-10m COMP$). We analyze node types and voting behaviors, which allows us to identify the different characteristics between whales and grassroots.
Figure~\ref{fig:c-2} shows $10$ clusters of CompoundDAO nodes, calculated based on their voting behavior and weight. %, which resulted from similar or different voting patterns. %for proposals. (while CompoundDAO contains voting labels for of 1 and -1 from $v-1$ to $v-90$ proposals). The nodes are %\yang{colored based  on the cluster they belong to? \tanusree{yes}} and \yang{the edges represent two nodes voted in the same proposal? \tanusree{correct}} 
Moreover, considering the information obtained from the CompoundDAO off-chain governance voting profile, we identify the ``type of organizations''. 
We color the nodes depending on their types, where green represents ``grassroot users,'' blue is ``industry,'' red is ``educational institute,'' and yellow is ``non-profit''. 
 %The ``grassroot users'' cluster represents addresses with token holding that is less than the whale address token threshold. 
 %\fixme{move this where grassroot first used}. 
From Figure~\ref{fig:c-2}, one can see that non-profit organizations tend to agree with the grassroot and broader communities regarding votes. The blue nodes ``industry'' tend to vote in a manner that are less likely to be people representative or have different voting patterns from ``grassroot.'' ``Education Institute'' seems to have similar voting patterns to ``industry.'' %\fixme{add quant value for different trend of whale voting}
% \yujin{Can we show the similar and different trends quantitatively? It is hard to see the above description from the figure alone.}
%\yujin{What do you mean by people representatives? If they have a similar voting behavior to grassroots users or most users, then we can say they are people representatives?} \tanusree{yes}
%In the next step, we separated the whale nodes and used the 4 categorizations (KOLs, industry, education industry, non profit organizations).  In the whale address cluster, we identified four main holders.

In Figure~\ref{fig:c-2}, 90.6\% of the green nodes have less than 0.25 tokens. From green nodes, we found a few users (don't represent any industry entity) having tokens in the whale threshold and have a certain influence in the CompoundDAO community (inferred from discourse conversation~\cite{comp}
%\yujin{We defined the grassroots mean non-whales above, right? What do you mean by grassroots users with many tokens?} \tanusree{there are few nodes which are not industry entity, rather individual}. 
Thus, we name them as ``\textbf{Key opinion leader} \footnote{A key opinion leader (KOL) is a trusted, well-respected influencer with proven experience and expertise, here in DAO community.}'' and presented those nodes with bigger thresholds of token weights.
%\yujin{We should move this to the above paragraph. Need to clarify the difference between grassroots and key opinion leaders in the above para. Or in figure~\ref{fig:c-2}, you didn't differentiate greenroots from key leader? If so, why you did so?} %\yang{light yellow?} \tanusree{its yellow} 
Figure~\ref{fig:c-3} shows graph connectivity (voting similarity) among nodes with significant delegated voting weight that is, whale addresses that fall into one of the following categories, ``Key Opinion Leader,'' ``Industry,'' ``Non-Profit,'' and ``Educational Institute''. 
These addresses significantly contribute to the CompoundDAO proposal's success (i.e., accept) or failure (i.e., reject). %in snapshot. 
%We also presented graph connectivity (voting similarity) of the whale addresses. 
%\tanusree{right now in 2(c)``Industry:blue,'' ``Non Profit:green,'' ``Educational Institute:red'', Key Opinion Leader:yellow'', but need to update the color to align with 2(b), so its consistent}
%351 are grassroot, 33 have more than 0.25 token
%Based on the information obtained from the CompoundDAO off-chain governance voting profile, we have found 34 whale addresses to be categorized into three main clusters: a) \textbf{industry} ; b) \textbf{Educational Institute} ; c) \textbf{Key Opinion Leader} (in Figure ~\ref{fig:c-3}), d) non-profit organization. 
%
The nodes are connected to each other via a different colored edge, depending on their similarity in voting behaviors. 
%pecifically, black edges represent the similarity of voting inside the same cluster/group of users, and red colored edges present the similarity of voting patterns among different clusters/groups of users. 
%
An address/node can represent a person or a group of people (of different autonomous organizations). However, due to the lack of user profiles (unlike CompoundDAO), it is hardly possible to differentiate the category of organization in many other DAOs we explored. 

%\yujin{I think I can revise the sentences from ``An address/node can represent...'' after seeing the different DAO results and their descriptions.} \tanusree{like compoundDAO, other DAOs doesn't have organization type available.}

%\korn{Key takeaway here would be helpful}

% \begin{tcolorbox}[width=\linewidth, colback=white!95!black, boxrule=0.5pt, left=2pt,right=2pt,top=1pt,bottom=1pt]
% \stepcounter{observation}
% {\bf Takeaways \arabic{observation}:}
% \fixme{add tanusree}
% }

% \end{tcolorbox}

\begin{comment}
\begin{table}[!htbp]
  \centering
%   \resizebox{\columnwidth}{!}
\fontsize{12pt}{30pt}
  \resizebox{1.0\linewidth}{!}
  {\begin{tabular}{l l l l l}
 \hline
DAOs &Vertics & Edge & Diameter&Mean Distance\\ 
 \hline
 BItDAO&60&932&4&1.50 \\ 
 CompoundDAO & 380 & 16147 & 3 & 1.78\\
 AssangeDAO &1017&516636& 7& 2.34 \\
 Proof of Humanity DAO &6035&100345&3&1.77\\
 BanklessDAO & \\
 KrauseHoueseDAO&\\
 \hline

  \end{tabular}}
  \caption{
  Network graph statistics for each DAO in terms of number of vertices, edges, diameter and mean distance.}
  \label{Tab:Tab1}
\end{table}



\begin{table}[!htbp]
  \centering
%   \resizebox{\columnwidth}{!}
\fontsize{12pt}{30pt}
  \resizebox{1.0\linewidth}{!}
  {\begin{tabular}{l l l l l}
 \hline
DAOs & Reciprocity & Transitivity & Assortativity\\ 
 \hline
 BITDAO& 1& 0.90&0.0045\\ 
 CompoundDAO &1& 0.59&	-0.22\\
 AssangeDAO &\\
 Proof of Humanity DAO &\\
 BanklessDAO & \\
 KrauseHoueseDAO&\\
 \hline

  \end{tabular}}
  \caption{Network Graph connectivity and clustering statistics for each DAOs in terms of reciprocity, transitivity and assortativity}
  \label{Tab:Tab2}
\end{table}

\end{comment}
% \begin{figure}
%   \includegraphics[width=1.0\columnwidth]{vote-network.png}
%   \caption{BitDAO user address in different proposal voting }
%   \label{fig:p1-pic}
% \end{figure}

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}

\subsection{DAO Holders' Proposal Pattern}
\label{proposal}
In this section, we analysed of DAO holders' proposal data to investigate the potential influence of various factors on proposal outcomes. 
%Specifically, we consider the author's address, their token holdings at the time of proposal creation, and the organizational category (if available) of the author (such as industry, educational institute, and general users) in relation to proposal success.
%\yang{I'd test the model: $outcome = token_amount + (1 | address)$} \tanusree{tested. will add the result soon} \tanusree{done and reported}
%\subsubsection{Procedure}

\subsubsection{Factors Influencing Proposal Outcome} 
\label{proposal-find}
We first performed logistic regression of the proposal outcome, where the predictor is the amount of token holdings of proposers at the time of the proposal. We statistically confirm if the amount of token holdings dictates the outcome of the proposal. 
%Based on the logistic regression analysis, we presented the probability of the proposal to be successful in 10 DAOs or not. We also considered possible contextual factors if needed. 
Second, we investigated the potential relationship between token holdings and proposal success. To this end, a mixed-effect regression analysis was conducted on the proposal outcome, with token amount as a fixed effect and id (address) as a mixed effect variable. The significance of this model was then evaluated using an ANOVA test, in comparison to a base model that only included id as a mixed effect and did not consider token amount as a fixed effect. This test was conducted under the assumption that \emph{token holdings may increase the possibility of success.} Additionally, we run another significance test for proposal outcome, comparing it to a base model that did not include id as a mixed effect, in order to investigate the potential influence of author address on proposal success. 
%The findings of this analysis is presented in the following section

%From this exploratory outcome and success rate of proposal, we form our Second hypothesis- 

% \begin{center}
% \begin{tabular}{||c ||} 
%  \hline
% \textbf{ H2}: Who the proposal author and Amount of  \\ token holdings predicts the
% outcome \\ of the proposal in DAOs. \\ 

%  \hline
%  \hline
% \end{tabular}
% \end{center}


% \tanusree{need to look into the proposals that tend to be failed and what happened after it failed. Is there any specific way DAO deals with the proposal that failed and improve that for next submission?? Especially will look deeper into the proposal from normal users that failed and the successive discussion in discourse channel to see if there is any pattern of discussion that might have something to do with the proposals' failure}
%\subsubsection{Findings}

%We report the probability of the proposal to be successful under the assumption that \textit{``the token amount dictates the proposal outcome.''}. 
We find a significant positive correlation between the \textit{\textbf{``token amount''}} and the proposal outcome (p-value<0.05) in CompoundDAO, dxDAO and krauseHouse,. In particular, for CompoundDAO, we find that token holdings have a significant effect ($p-value = 0.00676$) with an odd ratio of $95\% CI [1.244048, 1.000015]$. Further, the mix-effect analysis also confirms the token holding's significance to proposal success with the ANOVA test ($Pr(>X^{2}): >0.05$). 
%For some contextual information, we also present the proposal trend of CompoundDAO in Figure~\ref{fig:flow3} in Appendix. 
For contextual information, total 128 proposals submitted to CompoundDAO between May 1st, 2020 and December 5th, 2022 revealed that industry leaders and key opinion leaders (KOLs) were responsible for 101 of these proposals. Of these, 90\% were submitted by authors who held significant amounts of tokens. Overall, proposals submitted by organizations (e.g., Alameda Research)%, Polychain Capital,Gauntlet, Blck ) 
 and KOLs (e.g., Arr0)%Robert Leshner, , Getty Hill) 
had an aggregate success rate of 88.9\%. In contrast, proposals submitted by "grassroot users" had a success rate of 50\%.
%In terms of organizational success rates, non-profit organization Blck had a 100\% success rate with 20 proposals, followed by Gauntlet with 16 out of 18 successful proposals, Dharma with 6 out of 6 successful proposals, and Alameda Research and Polychain Capital with 3 out of 3 successful proposals. Other organizations and KOLs with high success rates included Robert Leshner, Arr0, GFX Labs, MonetSupply, Getty Hill, Nomic Foundation, Blockchain at Berkeley, Trail of Bits, and OpenZeppelin.
%\fixme{will move this to appendix if space needed} 

%In order to identify patterns of community interaction among proposal authors, we mapped author names and addresses to discussions on community forums and found that 11 addresses were particularly active in these forums (as shown in Figure ~\ref{fig:flow4}). We analyzed their engagement in discussions, including "soft proposals," and calculated the average frequency of conversation for each user. We also evaluated the level of engagement of each user based on their community contributions, responses, reading time of different posts, and engagement with community posts on Discourse. Figure ~\ref{fig:flow4} presents the average engagement level of these users on the x-axis and is color-coded according to their trust level \footnote{The trust level of each user is determined by the Discourse channels, which measure engagement and rate them in different trust level.}.
%\footnote{(green - Trust level Member, yellow: Trust Level basic members, red: Trust level 0 users). ``na: Trust Level 0'' implies new or not active in the community forum, trust yet to be earned; ``Level 1: Trust Level Basic User'' mostly reads community discussion, ``Level 2: Trust Level Member'' keeps coming back to the community over a series of weeks; they have not only read but also actively participated long and consistently enough to be trusted with a full membership.}. 

Similarly, dxDAO (p-value: $7.25e^{-07}$) and KrauseHouse (p-value: $0.00054$) also show the significance of token holdings to the proposal's success. The mixed effect analysis with the assumption of token holding to increase the proposal success possibility also confirms the significance for dxDAO ($Pr(>X^{2}): 0.01247$). Further, the mixed effect analysis with the assumption of author address to increase the proposal success possibility also shows the significance for dxDAO ($Pr(>X^{2}): 2.2e^{-16}$). On the other hand, we did not observe any significance of token holdings for BitDAO, BanklessDAO, and AssangeDAO.
However, there could be other contextual factors; for example, in BitDAO, there are predefined whitelisted addresses, and addresses that own more BIT than the proposal threshold (200000 BIT) can only propose.
%\korn{I tend to agree with this point, but maybe there is more to it as we can say the same thing for compound.}. 
Therefore, homogeneity across token holdings can limit model functionality. Furthermore, BitDAO shows a significant result ($Pr(>X^{2}): 2.2e^{-16}$) of \textit{\textbf{``author address''}} as a mixed effect to increase the possibility of proposal success. Similarly, for BanklessDAO, there are predefined authors selected to propose, while only the addresses from the consensus layer in AssangeDAO can propose. Proof of Humanity, Meta Gamma Delta, and MolochDAO where anyone can propose, showed no significance for \textit{``token holding''} with proposal success. 
%For PoH, everyone has equal number of token to vote. 
Although people can delegate their votes, the total vote is $1+\sqrt{delegated vote}$ for PoH having equal number of token to vote. For example, 16 addresses delegate to an address, then the total vote for that address would be $1+4=5$. This means there is some level of homogeneity across token holding. However, for Proof of Humanity ($Pr(>X^{2}): 2.2e^{-16}$) and Meta Gamma Delta ($Pr(>X^{2}): 1.02e^{-10}$), we found a significance of \textit{``author address''} to increase the possibility of proposal success.

% \begin{figure*}
%   \includegraphics[width=2.0\columnwidth]{bit-gov.pdf}
%   \caption{BitDAO Governance structure with both off-chain and on-chain activities and requirements/main components \tanusree{will update this with comparative model for 5 DAOs side by side to show the difference on infrastructure use}}
%   \label{fig:p2-pic}
  
% \end{figure*}
\begin{tcolorbox}[width=\linewidth, colback=white!95!black, boxrule=0.5pt, left=2pt,right=2pt,top=1pt,bottom=1pt]
\stepcounter{observation}
{\bf Takeaways \arabic{observation}:}
{Proposal success has a significant positive correlation with token holdings by proposers for KrauseHouse, CompoundDAO, and dxDAO. However, BitDAO, BanklessDAO, and AssangeDAO showed no significant correlation due to predefined whitelisted authors.
}

\end{tcolorbox}


\subsection{DAO Holders’ Voting Power}

In this section, we estimate the decentralization level regarding holders' voting power.

\subsubsection{Evaluation of Decentralization Levels}

%\noindent {\bf Correlation Analysis.} 
First, we conducted a correlation analysis between voters' token weight and a participation rate, which is defined as the number of proposals that a voter participated in. We aim to determine whether the participation rate, therefore the voting power, is biased toward rich token holders. Here, the positive correlation between the participation rate and token weight may imply worse decentralization due to the more active participation of only richer voters than the others. Table~\ref{tab:decen-level} summarizes a Pearson correlation coefficient and p-value of 10 DAOs. While the results were mixed, five systems - CompoundDAO, BitDAO, AssangeDAO, Proof of Humanity, and LivePeer - showing a significant positive correlation. MetaGammaDelta, on the other hand, displayed a significantly strong negative correlation. Consequently, it appears that in many DAOs, wealthy voters are more likely to participate, exacerbating poor decentralization.

%Many DAO systems show a positive correlation; five DAOs, CompoundDAO, BitDAO, AssangeDAO, Proof of Humanity, and LivePeer, show a significant positive correlation, MetaGammaDelta shows a significantly strong negative correlation, and the analysis for the others results in an insignificant or negligibly weak correlation. As a result, in many systems, rich voters tend to participate more than poor voters, aggravating poor decentralization.

\begin{table*}[]
%\scriptsize
\small
\begin{tabular}{lllllllll}
\hline
Name              & Corr. & P-value   & \begin{tabular}[c]{@{}l@{}}Entropy \\ (Token)\end{tabular} & \begin{tabular}[c]{@{}l@{}}Entropy\\ (Voting score)\end{tabular} & \begin{tabular}[c]{@{}l@{}}Gini\\ (Token)\end{tabular} & \begin{tabular}[c]{@{}l@{}}Gini\\ (Voting score)\end{tabular} & Nakamoto & \begin{tabular}[c]{@{}l@{}}The num. \\ of voters\end{tabular} \\
\hline
CompoundDAO       & 0.27  & 3.32E-44  & 5.86                                                       & 5.17                                                             & 0.98                                                   & 0.99                                                          & 15       & 2483                                                          \\
BitDAO            & 0.21  & 0.0005    & 3.9                                                        & 3.35                                                             & 0.96                                                   & 0.97                                                          & 6        & 284                                                           \\
AssangeDAO        & 0.24  & 4.69E-15  & 7.83                                                       & 7.42                                                             & 0.84                                                   & 0.87                                                          & 50       & 1066                                                          \\
Proof of Humanity & 0.38  & 2.18E-108 & 11.46                                                      & 8.85                                                             & 0.05                                                   & 0.73                                                          & 1448     & 3086                                                          \\
Bankless DAO      & 0.05  & 0.003     & 9.95                                                       & 9.13                                                             & 0.7                                                    & 0.84                                                          & 268      & 3234                                                          \\
KrauseHouse       & 0.05  & 0.15      & 5.59                                                       & 4.68                                                             & 0.91                                                   & 0.95                                                          & 7        & 592                                                           \\
LivePeer          & 0.5   & 3.57E-27  & 5.36                                                       & 4.63                                                             & 0.91                                                   & 0.95                                                          & 9        & 368                                                           \\
MetaGammaDelta    & -0.89 & 1.99E-07  & 4.22                                                       & 3.62                                                             & 0.03                                                   & 0.51                                                          & 9        & 19                                                            \\
MolochDAO         & 0.18  & 0.51      & 2.37                                                       & 1.823                                                            & 0.73                                                   & 0.81                                                          & 2        & 15                                                            \\
dxDAO             & 0.03  & 0.57      & 6.21E-12                                                   & 1.25E-11                                                         & 0.99                                                   & 0.99                                                          & 1        & 278     \\
\hline
\end{tabular}
\caption{Evaluation of decentralization levels through correlation analysis and three metrics: Entropy, Gini coefficient, and Nakamoto.}
\label{tab:decen-level}
\end{table*}

\begin{figure*}[!htb]
\begin{subfigure}{0.45\textwidth}
  \includegraphics[width=\linewidth]{images/compound.pdf}
  \caption{CompoundDAO Decentralization Level Overtime}\label{fig:decen-level1}
\end{subfigure}\hfill
\begin{subfigure}{0.45\textwidth}
  \includegraphics[width=\linewidth]{images/poh.pdf}
  \caption{Proof of Humanity: Decentralization level over time }
  \label{fig:decen-level2}
\end{subfigure}
\caption{Voting Power Evaluation of decentralization level by Entropy, Gini coefficient, and Nakamoto showed significantly poor decentralization for Compound, BitDAO, Krasehouse, MolochDAO, and dxDAO while the highest decentralization level for Proof of Humanity. Unlike many DAO systems including CompoundDAO, the decentralization level of PoH is in increasing trend over time.}
\label{cluster2}
\end{figure*}
  
%\noindent  {\bf Evaluation of decentralization levels} 
Next, we evaluated decentralization level of 10 DAOs in terms of the voting power. To do this, we used three metrics: Entropy, the Gini and Nakamoto coefficient. Entropy can be generally used to assess randomness and degrees of freedom for a given system. Mathematically, the metric for given a series of numbers $x (={x_i})$ is defined as follows: 
$$\vspace{-2mm}Entropy(x)=\sum_{i}log_2\left(\frac{x_i}{\sum_{i}x_i}\right)*\frac{x_i}{\sum_{i}x_i}.\vspace{-2mm}$$ 
If the value of entropy is high, it implies a DAO has a high degree of randomness and freedom, which is related to a high level of decentralization. The Gini coefficient used to measure the wealth inequality traditionally can be applied to assess the voting power inequality among voters in our analysis. The metric for given a series of numbers x is defined as follows: 
$$\vspace{-2mm}Gini(x)=\frac{\sum_{i,j}|x_i-x_j|}{2 |x| \sum_{i}x_i},$$ 
where $|x|$ indicates the length of the number series. The minimum value of the Gini coefficient as 0 would represent the full equality among voters, while the maximum value of 1 would represent the full power bias towards one voter. We calculated Entropy and Gini based on the token weight of voters and their voting scores, which, in this paper, we define as \textit{``token weight$\times$the number of proposals that a voter participated in''} to reflect not only the token weight but also a participation rate. Lastly, the Nakamoto coefficient indicates the minimum number of entities that can subvert the system. In the voting context, the entities can accept or reject the proposal in accordance with their interests, even if it may be against most users. Therefore, if power is significantly biased towards only a few voters, the DAO cannot be considered to attain true democracy, which is one of the main goals of DAOs. We calculated the Nakamoto coefficient based on the token weight of voters.    

From Table~\ref{tab:decen-level}, we can see almost all DAOs suffer from poor decentralization. In particular, Compound, BitDAO, Krasehouse, LivePeer, Meta Gamma Delta, MolochDAO, and dxDAO showed significantly poor decentralization, where their Gini coefficients were above 0.9 due to a extremely large power inequliaty or (and) the Entropy values were low due to a low number of participating voters. On the other hand,  Proof of Humanity showed the highest decentralization level among our target DAOs. In fact, it uses one-person-one-vote protocol unlike the popular protocol that the voting power is proportional to token amounts holded by a voter. However, note that our result analysis does not necessarily mean that one-person-one-vote protocol is better than the other protocol using the token capital concept; even though Meta Gamma Delta also uses a similar protocol to Proof of Humanity, it currently suffers from the low number of active voters. 

\begin{tcolorbox}[width=\linewidth, colback=white!95!black, boxrule=0.5pt, left=2pt,right=2pt,top=1pt,bottom=1pt]
\stepcounter{observation}
{\bf Takeaways \arabic{observation}:}
{In many DAOs, richer token holders tend to participate more actively in the voting process, which aggravates the decentralization of the voting process. Moreover, almost all DAOS that we analyzed are suffering from poor decentralization. 
}

\end{tcolorbox}


\subsubsection{Decentralization Dynamics Overtime} 

We also present the decentralization dynamics over time. Table~\ref{tab:decen-over} in Appendix summarizes the linear regression results of 10 DAOs, where we mark significantly negative and positive decentralization trends with red and blue, respectively. Overall, we can see that many DAOs (CompoundDAO, BitDAO, AssangeDAO, BanklessDAO, and KrauseHouse) show a significantly negative decentralization trend: the decreasing decentralization level over time (Figure~\ref{fig:decen-level1}). On the other hand, Proof of Humanity and MGD have a significantly positive decentralization trend: the increasing decentralization level over time (Figure~\ref{fig:decen-level2}). Note that, according to Table~\ref{tab:decen-level}, in the Proof of Humanity system, a biased participation rate of voters is more a matter rather than a biased token weight distribution  in terms of a decentralization level; entropy and the Gini coefficient for voters’ token weight are high and low, respectively. Therefore, we focus on the linear regression result for Entropy rather than that for the Gini coefficient shown in Table~\ref{tab:decen-over}. One can find that both DAOs, Proof of Humanity and MGD, are a system adopting the one-person-one-vote protocol. As a result, the level of decentralization has got better over time in the one-person-one-vote protocol. 

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}


\begin{tcolorbox}[width=\linewidth, colback=white!95!black, boxrule=0.5pt, left=2pt,right=2pt,top=1pt,bottom=1pt]
\stepcounter{observation}
{\bf Takeaways \arabic{observation}:}
{The decentralization dynamics analysis shows that decentralization has been gradually aggravated in a voting protocol based on token capital, while it has improved over time in the one-person-one-vote protocol.
}

\end{tcolorbox}
\begin{comment}
\subsection{Gas Cost to Participate in Voting}
\subsubsection{Cost to Participate}

In order to evaluate overall participation across different DAOs, this study analyzed the cost of proposing, delegating, and voting in each DAO in USDT/ETH over time (from the time of their formation to December 5th). It is important to note that off-chain voting typically has no cost associated, Therefore, this analysis focuses on on-chain DAOs: CompoundDAO, MGD, Moloch, dxDAO, and LivePeer.

\begin{table}
    \centering
 \small
%\fontsize{12pt}{30pt}
  \resizebox{1.0\linewidth}{!}
  {\begin{tabular}{l l l l l}
 \hline
DAO & Propose (USDT) & Propose (Gas Used) & Vote (USDT) & Vote (Gas Used)\\ 
 \hline

Compound&100.75&729865.78&3.95&75866.48\\
MGD& 20.42 & 424970.0&3.91&99866.98\\
Moloch &77.06&529194.69&16.32&103001.61\\
dxDAO &23.43&444954.687&6.59&285786.24\\
LivePeer&19.75&198149.00&1.63&46780.28\\
 \hline

  \end{tabular}}
  \caption{Overview of the average gas cost in ETH to participate in each DAO. Rows are DAOs. Columns are average costs to Propose/Vote/Delegate in ETH/USDT}
  \label{Tab:Tab-gas-cost}
\end{table}



We notice each DAO to be optimized for different functionality, which results in heterogeneous smart contract implementations. This also implies a different gas cost to participate across DAO systems because the ``Gas Used'' unit depends on smart contract implementation. For example, Livepeer has the simplest implementation for an on-chain voting system, providing the lowest cost for both proposing and voting among the five on-chain DAOs. CompoundDAO has the highest cost to propose while having a relatively low voting cost compared to other DAOs.
This encourages many users to participate in the voting process, which enables the system to satisfy a high quorum value (refer to Table~\ref{tab1:macro}). 
On the other hand, dxDAO, Moloch, and MetaGammaDelta are the most expensive to vote on a proposal. This can prevent many users from participating in the voting protocol. 
Given this, for MetaGammaDelta and MolochDAO, a typical proposal does not have a quorum; that is, they can decide on an outcome of a proposal without requiring the minimum number of addresses that should vote. Similarly, for dxDAO, if the proposal has been sponsored, there are no quorum requirements.


\subsubsection{Cost to participate(vote) vs. Participation Ratio/Decentralization}
We conducted a correlation analysis between the gas cost to vote (USDT) and the decentralization level. To do this, for each DAO proposal, we considered the average gas cost and three decentralization metric values (entropy and the Gini coefficient based on voters’ token weight and the number of voters). 

\begin{table}
    \centering
 
\fontsize{12pt}{30pt}
  \resizebox{1.0\linewidth}{!}
  {\begin{tabular}{l l l l l}
 \hline
DAO & Gas-Entropy (token) & Gas-Gini (token)&Gas-# of voters\\ 
 \hline

Compound&0.3065 (0.0004) &-0.2827 (0.0012)&-0.1055 (0.2343)\\
dxDAO &-0.3329 (1.2825e$\small ^{-27}$)&-0.2968 (5.0207e$^{-22}$)&-0.2625 (2.0734e$^{-17}$)\\
LivePeer&0.2943 (0.5712)&0.1052 (0.8427)&0.2612 (0.6172)\\
MGD&-0.1289 (0.2875)&0 (0)&-0.1289 (0.2875)\\
Moloch&-0.1014 (0.6297)&-0.1768 (0.3979)&-0.0035 (0.9866)\\
 \hline
  \end{tabular}}
  \caption{Correlation Result: Cost to participate (vote) vs. Participation Ratio/Decentralization over time}
  \label{Tab:Tab-gas-cost1}
\end{table}

The correlation results are mixed depending on the DAO system. CompoundDAO shows a significant correlation for entropy and the Gini coefficient. Specifically, its result implies that it is more likely to have a higher decentralization level (i.e., higher entropy and a lower Gini value) under a higher gas fee; as costs increase, the degree of randomness for the voting system increases, and token distribution among voters tends to be more uniform. 
Similarly, dxDAO also shows a significant negative correlation between the Gini coefficient and gas costs. It supports a connection between a higher decentralization level and a higher gas fee. On the other hand, the correlation results for the entropy and the number of voters support the other direction. As a result, in a higher gas cost regime, one can see that the token weight distribution becomes more uniform, but more users with low token balances do not participate in the DAO voting system, which leads to a decrease in the overall decentralization level. This is opposite to the result of CompoundDAO showing the connection between a higher overall decentralization level and a higher gas fee. On the other hand, other DAO systems do not have significance for the correlation analysis. 

\begin{tcolorbox}[width=\linewidth, colback=white!95!black, boxrule=0.5pt, left=2pt,right=2pt,top=1pt,bottom=1pt]
\stepcounter{observation}
{\bf Takeaways \arabic{observation}:}
{
The correlation between the decentralization level and the gas fee to vote is inconsistent; if a gas cost becomes higher, CompoundDAO tends to be more decentralized, while dxDAO tends to be less decentralized. 
Therefore, there should be other factors that determine a decentralization level of a DAO voting system.
}

\end{tcolorbox}
\end{comment}

\vspace{-2mm}
\section{RQ3: Autonomy of DAOs}
\vspace{-2mm}
\label{section6}
%  --- I think 7.1 would be better off removed as arbitrary tx execution has little to do with autonomy
%  --- 7.2 I think is not well framed, since an autonomous organization that "hires" a third party to carry out is still autonomous if it retains the ability to e.g., make payment conditional on whether the third party has succeeded. Maybe a framing can be about how much power DAOs give to the third parties once they are hired?
%  --- 7.3 the examples here I don't think relate to autonomy. When the multisig of a DAO overrides the broader voting process, this is a decentralization issue, not an autonomy issue, since the multisig is still internal to and part of the DAO rather than external.
%  --- Some better examples of autonomy failure would be DAOs could be the censorship that was seen on Ethereum due to OFAC sanctioning of Tornado cash, or potentially any other regulator actions.

%Next, we evaluate the autonomy of 10 DAOs. 
%While there exists many angles to evaluate the level of autonomy of a DAO, such as financial and legal autonomy, we aimed to explore the DAO's autonomy from the angle of governance proposal.
%\korn{is there a better term than 'proposal processing'?}
For the DAO autonomy analysis, we explore (1) whether a DAO system can execute arbitrary transactions, (2) whether it relies on third parties after transaction execution, and (3) whether proposals have been canceled after being successful. %, and (4) how long they were delayed to be executed.
\vspace{-2mm}
\subsection{Capability of Arbitrary Transaction Execution}
\vspace{-2mm}
%\noindent The ability to execute arbitrary transactions is a crucial aspect of DAOs~\cite{das2019fastkitten}.
Arbitrary transaction execution refers to the capability of a DAO to fulfill various proposals, regardless of their specific requirements. Without this capability, a DAO's functionality is limited, requiring additional intervention to execute certain transactions on-chain, like transferring funds to an EOA\footnote{Externally Owned Account (EOA) refers to addresses that are managed by a private key and not a smart contract code.} to carry out proposal execution. This would decrease the DAO autonomy. To achieve arbitrary transaction execution, DAOs should interact with any contract %on the same blockchain 
by passing call data through the call function in Solidity~\cite{das2019fastkitten}. 

To determine the capability of a DAO to execute arbitrary transactions and related methods, 
%by which it does so, 
we first thoroughly examined the smart contracts listed on the DAO's website or Github repository. 
Specifically, we searched for code snippets that enable arbitrary transaction execution. 
%To ensure that the code snippets are used in deployment, we verify them against smart contract source codes on Etherscan used in DAO proposal execution transactions.
%We then identified the treasury address of the DAO and
%through the information available on their website and their voting platform (such as Snapshot, DAOHaus, etc.). 
%traced transactions from the treasury address to proposals through the voting platform and located the address of the code snippet we had previously identified, thus validating the DAO's use of a contract with arbitrary transaction execution capability\tanusree{@korn, can this earlier line be concise? its hard to read and understand.}. 
%We also analyzed the smart contract codes of the DAOs and how they interact with other entities on the blockchain. 
% Figures~\ref{fig:code-snippet-1} and \ref{fig:code-snippet-2} in Appendix provide examples of different types of arbitrary transactions, including on-chain\footnote{The transaction list is crafted at proposal submission and queued in timelock or executed right after voting, all processes are done on-chain, and no one can stop this (except the proposer in some cases).}, multisig\footnote{Core members craft a list of transactions for a particular proposal and execute them on the chain with a multisig}, and Kleros Governor contract\footnote{Anyone can craft a list of transactions satisfying the proposals, and community member double check on the crafted list and can challenge the list.} 

Our study indicates that 10 DAOs have protocols for executing arbitrary transactions, albeit with varying autonomy levels. Table~\ref{Tab:Tab-auto-met-1} in Appendix summarizes the protocols used in executing arbitrary transactions.
Most DAOs that employ on-chain voting, including CompoundDAO, Meta Gamma Delta, Moloch, and dxDAO, exhibit an entire pipeline for voting, consensus building, and execution. Consequently, we find such DAOs to be most autonomous, as the transaction sequence is determined upon proposal submission and immutable thereafter. Conversely, DAOs employing off-chain voting necessitate a means of transposing the off-chain consensus onto the on-chain ledger, such as multisig wallet to issue on-chain transactions. Most off-chain voting DAOs, including AssangeDAO, BitDAO, Banklass, and KrauseHouse, and LivePeer use a multisig wallet to issue on-chain transactions. Multisig lowers decentralization and autonomy levels, as a small group wields controls over the on-chain actions to be executed, however, eases the implementation and maintenance. 
%Another method to bring transactions on-chain is to allow individuals to propose a list of transactions to fulfill approved proposals, which will then be executed after a period of time. In the event that someone submits a competing list of transactions, a community dispute arises, and the winning transaction list gets rewarded from the losing list's stake. 
Alternately, on-chain transactions to fulfill approved proposals can be crafted and refined by community members through a system of checks and balances involving monetary stakes.
Kleros Governor contract~\cite{kleros} exemplifies this approach, which is adopted by Proof of Humanity. Although this method is more decentralized than a multisig wallet, it still limits autonomy, as multiple parties must verify %the validity of 
the proposed transactions list, which, but, would delay execution. 
%
Figures~\ref{fig:code-snippet-1} and \ref{fig:code-snippet-2} in Appendix provide examples of code snippets for different types of arbitrary transactions, including on-chain
%\footnote{The transaction list is crafted at proposal submission and queued in timelock or executed right after voting, all processes are done on-chain, and no one can stop this (except the proposer in some cases).}
and multisig. 
%\footnote{Core members craft a list of transactions for a particular proposal and execute them on the chain with a multisig}
%\footnote{Anyone can craft a list of transactions satisfying the proposals, and community member double check on the crafted list and can challenge the list.} 

\begin{tcolorbox}[width=\linewidth, colback=white!95!black, boxrule=0.5pt, left=2pt,right=2pt,top=1pt,bottom=1pt]
\stepcounter{observation}
{\bf Takeaways \arabic{observation}:}
{
%The approach to achieve arbitrary transaction execution varies among the DAOs, with having the transaction data included at proposal submission on-chain being the most autonomous. 
DAOs vary in their approach to executing arbitrary transactions, with fully on-chain pipeline being the most autonomous.
Multisig approach trades autonomy for simplicity, while Kleros contract also lacks autonomy even though it increases decentralization. % in bringing off-chain consensus on-chain.
}
\end{tcolorbox}

\vspace{-3mm}

\iffalse
\subsubsection{Execution Time Delay}
%Part of being autonomous is the ability of a DAO to promptly translate consensus into actions. 
%Execution time delay indicates the time between a transaction being executable to the actual execution time.
%For the execution time delay analysis, we collected proposal timeline data, including Timestamps of proposal execution and proposal voting ends. 
%and analyze whether the proposal time delay is correlated with a gas cost.
%When comparing the average execution time delay of the
Out of 10 DAOs, CompoundDAO has the lowest at 4h 58 min  (Figure~\ref{fig:time-delay}). It %CompoundDAO is one of the most popular DAOs and 
has its proposal pipeline entirely on-chain.
%and their proposals are more urgent in general (e.g., updating parameters, new token support, new functionality) than a proposal on other DAOs (e.g., membership, grant request, etc.) 
On the other hand, MetaGammaDelta has the highest execution time delay with 5d 15h 23 min on average, likely due to its smaller number of active participators than other DAOs.
%and most proposals are on membership approval, which is not an urgent matter.
\begin{figure}[!t]
\centering
\includegraphics[width=\columnwidth]{images/compound_exe_time_delay.png}
\caption{Average execution time delay for CompoundDAO proposal over time}
\vspace{-5mm}
\label{fig:time-delay}
\end{figure}
\fi

% \begin{figure}[!t]
% \centering
% \includegraphics[width=\columnwidth]{images/mgd_exe_time_delay.png}
% \caption{Average Execution time delay for proposal in MetaGammaDelta Overtime}
% \label{fig:flow-dia-1}
% \end{figure}

% \begin{tcolorbox}[width=\linewidth, colback=white!95!black, boxrule=0.5pt, left=2pt,right=2pt,top=1pt,bottom=1pt]
% \stepcounter{observation}
% {\bf Takeaways \arabic{observation}:}
% {
% It is observed that the execution time delay varies from 4 hours up to 6 days for on-chain DAOs. 
% %Also, we find that there is little correlation between gas price and execution delay. %High average gas price can be one of many factors positively impact the length of delay, which may be more apparent in DAOs with smaller treasuries. 
% }
% \end{tcolorbox}
\vspace{-2mm}
\subsection{Third Party Dependency in Proposals}
\vspace{-2mm}
In DAOs, the reliance on external entities to fulfill proposals after the voting period is commonly known as third-party dependencies.
%In DAOs, third-party dependencies refer to the reliance on external entities to fulfill a portion of a proposal after it has passed the voting period. 
This reliance can imply lower DAO autonomy (please see Sections~\ref{subsec:rw-autonomous} and \ref{interview}), introducing uncontrollable external factors.
We investigate how current DAOs utilizing third-party services handle and minimize associated risks. Analyzing the relationship between DAOs and third parties can not only aid in evaluating autonomy but also provide insight into how DAOs currently benefit from third-party services, minimizing risk exposure. 
%For example, actions in CompoundDAO or BitDAO are considered third-party dependent if they are not proposed through the DAO's governance or executed through its designated contract (e.g. Timelock contract or Multisig). 
Third party dependent proposals are defined as those relying on other entities apart from the DAO itself to fulfill a part of the proposal after passing the voting period.
%We find that 
These proposals include payment for future services or delegating decision-making power to a small group. 
%These proposals rely on third-party services after their execution as the DAO is delegating trust to fulfill promises.
%
% 
%
%Third-party dependencies of a proposal means that a proposal needs to rely on a third party to fulfill a part of the proposal after after passing the voting period. Having reliance on 3rd party services after proposal consensus is reach  can be a sign of DAOs with lower autonomy as relying on a third-party service can bring an uncontrollable external factor. It is also important to investigate how the current DAOs that use the third-party service handle and minimize the risks. 
%Therefore, our analysis of the relationship between DAOs and third parties can not only help evaluate autonomy, but also provide an insightful hint on how DAOs currently benefit from third parties while minimizing risk exposure. 
%Third-party actions can be anything not originating from the DAO’s proposal pipeline. For example, in the case of CompoundDAO, an action would be considered as one made by a third party if it has not been proposed through the DAO governance or not executed through Compound’s Timelock contract. For BitDAO, an action can be considered as one made by a third party if it has not been proposed through the DAO governance or not executed through the DAO Multisig. \korn{add some examples} Some examples of third party dependent proposals after execution would be payment for some future services for the DAO or delegating some power to a small group of people to make future decisions for the DAO. The moment of proposal execution are setting up the payment and delegating the power respectively for the two examples, which means such proposals depends on 3rd party after execution.
% We sought to investigate the utilization of third-party services following the execution of proposals within DAOs. 
To investigate the utilization of third-party services, we analyzed both the content of proposals and associated execution data. Our evaluation process involved assessing the primary objectives of proposals to identify any post-execution intervention or deviation from the proposal's promises that could potentially negate the effectiveness or have a detrimental effect on DAOs.

%We identified the proposal that relies on third party services after its execution for each DAO by looking into the proposal content and the proposal execution data.
%To decide if a given proposal needs a third party after the execution, we considered the following: (1) What is the main goal of the proposal?, and (2) after execution, can someone intervene or break any promises made in the proposal to make the proposal void or make the DAO worse off?


Table~\ref{tab:3rd-party} presents the percentage of third party dependent proposals for nine different DAOs. dxDAO is left out of the analysis due to the large number of proposals making it infeasible to conduct the manual analysis. Of the 9 DAOs examined, only MetaGammaDelta DAO proposals do not rely on third-party services after execution because they are typically requests for membership or funding, with no return promises. The DAO with the highest percentage of third party dependent proposals is KrauseHouse ($74.81\%$). Many KrauseHouse proposals involve funding requests from third parties with commitments of future returns in the form of working hours.
While third-party reliance following proposal execution can be beneficial in allowing a DAO to achieve various goals, particularly those that are off-chain, DAOs should take measures to minimize the risks associated with third-party services. Our analysis identified strategies used by DAOs to mitigate these risks--(a) using stream payments instead of upfront lump sum payments, (b) using milestone-based payments where funds are paid based on completed tasks, and (c) assigning a committee with a multisig wallet to manage funds allocated for third-party.


\begin{tcolorbox}[width=\linewidth, colback=white!95!black, boxrule=0.5pt, left=2pt,right=2pt,top=1pt,bottom=1pt]
\stepcounter{observation}
{\bf Takeaways \arabic{observation}:}
{
Most DAOs require services from third parties to operate with common case is employment for some future services. 
%DAOs that have complicated offchain goals, such as KrauseHouse buying an NBA team, can have more reliance on third party. 
Despite such necessity of third parties in DAOs, there are many strategies to minimize the risk of third-party reliance.
}
\end{tcolorbox}
\vspace{-2mm}
\subsection{Proposals Canceled after Voting Ends}
\vspace{-2mm}
%We then examined proposals that were canceled after the voting period ended. These are proposals that were accepted but ultimately not implemented. 
Subsequently, we examined proposals that were accepted but not implemented, referred to as \emph{``canceled proposals.''} 
This measure serves as a proxy for evaluating whether community consensus is respected and whether a DAO is truly autonomous, i.e., whether a small group of individuals can prevent a DAO action from being carried out. 
%To determine the percentage of proposals that were canceled without execution, 
We analyzed events from the smart contracts of on-chain DAOs, except for LivePeer. For off-chain DAOs 
%and LivePeer, 
we manually examined data from Snapshot and Discourse to determine if the proposals have been successfully implemented.

%Table~\ref{tab:canceled} in Appendix shows our analysis result. 
Meta Gamma Delta, MolochDAO, and dxDAO have a ``binding'' consensus, indicating proposals are executed after acceptance through a smart contract, with no cancellation mechanism after the proposal has passed. Only 2 on-chain DAOs, CompoundDAO and Livepeer have a formal cancellation mechanism after the proposal has passed (Table~\ref{tab:canceled} in Appendix). In CompoundDAO, proposal cancellation can be done by the proposal author or by anyone if author's governance token balance drops below proposal threshold.
The proposals that were canceled after the voting period ends in CompoundDAO are mostly those overwritten by another proposal because of parameter/transaction issues~\cite{compound} and ones for a temporary bug fix ~\cite{compound1}. In the case of LivePeer, DAO requires a multisig to issue the transaction, and not everything is done on-chain. Thus, after the consensus is reached, multisig still can \emph{``cancel''} the proposal if they wish. For the remaining off-chain DAOs, proposals can technically be censored as off-chain consensus is not guaranteed to be brought on-chain. However, some off-chain DAOs still hold a binding consensus ideology. 
%and have not yet censored any proposals. 
While the percentage of proposals canceled is an important metric for autonomy, difficulty arises when empirically calculating this metric due to the limited transparency of the proposal status after consensus is reached in many off-chain DAOs.
%\yujin{How about the others? Why do they have a canceled proposal?} \korn{done}

\begin{tcolorbox}[width=\linewidth, colback=white!95!black, boxrule=0.5pt, left=2pt,right=2pt,top=1pt,bottom=1pt]
\stepcounter{observation}
{\bf Takeaways \arabic{observation}:}
{
Our data on the number of proposals canceled after voting ends suggests that DAOs tend to follow proposal binding ideology even if it is not guaranteed programmatically. A high number of unknown status proposals suggests that there is a need for proposal transparency tools.
}
\end{tcolorbox}



\begin{comment}


\begin{table}[]
\scriptsize
\centering
\begin{tabular}{cc}
\hline
DAOs  & Corr. (p-value) \\
\hline
CompoundDAO & -0.0039 (0.9685)\\
dxDAO & 0.0390 (0.3112)\\
LivePeer & -0.5492 (0.2017)\\
MetaGammaDelta & 0.1966 (0.1054)\\
MolochDAO & -0.1030 (0.6242)\\
\hline
\end{tabular}
\caption{The correlation coefficient between execution time delay and gas price (in ETH).}
\label{tab:delay_gas}
\end{table}

Moreover, we conducted a correlation analysis between gas price (in ETH) and execution time delay. Table~\ref{tab:delay_gas} shows the correlation coefficients for five on-chain DAOs. 
As a result, all DAOs do not have a significant correlation between gas price and execution time delay, implying little relationship between the two parameters. 
\end{comment}
%On the other hand, there is a positive correlation between the gas price and execution time delay for MetaGammaDelta and a negative correlation in LivePeer. 
%For LivePeer, the correlation analysis should be taken lightly as there are only seven proposals and the proposals require multiple transactions to fulfill over a period of time. MetaGammaDelta having the smallest treasury could be one of the reasons that there is a positive correlation as the cost to process a transaction relative to treasury size is larger compared to other DAOs.
%\yujin{Need to elaborate this more...} \korn{done: elaborated on why small treasury could be a reason}


\begin{table}[]

\begin{tabular}{lll}
\scriptsize

Name              & 1 (not reliance) & 0 (reliance) \\
\hline
AssangeDAO        & 81.81\%          & 18.18\%      \\
CompoundDAO       & 83.94\%          & 16.06\%      \\
BitDAO            & 72.22\%          & 28.78\%      \\
Proof of Humanity & 86.54\%          & 13.46\%      \\
Bankless DAO      & 70.59\%          & 29.41\%      \\
KrauseHouse       & 25.19\%          & 74.81\%      \\
LivePeer          & 85.71\%          & 14.29\%      \\
Meta Gamma Delta  & 100\%            & 0\%          \\
MolochDAO         & 84.84\%          & 15.15\%    \\
\hline
\end{tabular}
\caption{Percentage of proposals that relies on third-party services after execution. Rows are each DAOs where 0 means relying on a third party and 1 is not reliance}
\label{tab:3rd-party}
\end{table}
